Near-Optimal Communication Byzantine Reliable Broadcast under a Message Adversary

We address the problem of Reliable Broadcast in asynchronous message-passing systems with $n$ nodes, of which up to $t$ are malicious (faulty), in addition to a message adversary that can drop some of the messages sent by correct (non-faulty) nodes. We present a Message-Adversary-Tolerant Byzantine Reliable Broadcast (MBRB) algorithm that communicates ${\cal O}(|m|+n\kappa)$ bits per node, where $|m|$ represents the length of the application message and $\kappa=\Omega(\log n)$ is a security parameter. This communication complexity is optimal up to the parameter $\kappa$. This significantly improves upon the state-of-the-art MBRB solution (Albouy, Frey, Raynal, and Ta\"iani, TCS 2023), which incurs communication of ${\cal O}(n|m|+n^2\kappa)$ bits per node. Our solution sends at most $4n^2$ messages overall, which is asymptotically optimal. Reduced communication is achieved by employing coding techniques that replace the need for all nodes to (re-)broadcast the entire application message $m$. Instead, nodes forward authenticated fragments of the encoding of $m$ using an erasure-correcting code. Under the cryptographic assumptions of threshold signatures and vector commitments, and assuming $n > 3t+2d$, where the adversary drops at most $d$ messages per broadcast, our algorithm allows at least $\ell = n - t - (1 + \epsilon)d$ (for any arbitrarily low $\epsilon> 0$) correct nodes to reconstruct $m$, despite missing fragments caused by the malicious nodes and the message adversary.

==> correctnessAnalysis.tex <==
\section{Correctness analysis}
\label{sec:correctness}
We now analyze \cref{alg:3.1:merkle:trees} and show it satisfies the MBRB properties specified in
\cref{def:mbrb}. 
This analysis, along with the communication analysis in \cref{lem:communication} prove our main Theorem~\ref{thm:main-inf}.
\begin{theorem}
	\label{thm:main}
	For any network that satisfies \cref{asm:MBRBassumptionR} and for any $\eps>0$, 
	\Cref{alg:3.1:merkle:trees} implements an MBRB algorithm (\cref{def:mbrb}) with $\ell>n-t-(1+\eps)\Dadv$. 
 %A single activation of the algorithm on the input message~$m$ communicates $4n^2$ messages, where each node communicates $O(|m|+n^2\kappa)$ bits overall.
\end{theorem}

Recall that any MBRB algorithm requires $n>3t+2\Dadv$ \cite{AFRT23}. Our coded MBRB algorithm uses an error-correction code that can reconstruct any encoded message from $k$ fragments of the codeword. 
%
While we have some flexibility in selecting the value of~$k$, which affects the parameters of the ECC and thus the communication complexity,
%(\cref{sec:ECC-instantiation}), 
our proof requires that $k$ will not be too large. 
We therefore  assume the following throughout the analysis:
\begin{assumption}[coded-MBRB-assumption]
	\label{asm:MBRBassumptionR}
	$n>3t+2\Dadv$ and $\ECCthreshold\leq (n-t)-2\Dadv$.
\end{assumption}	
%\ran{Is the constraint on $k$ inherent? To me, it seems to follow since we assign 1 fragment per node, then dropping $\Dadv$ messages immediately means $k<n-t-\Dadv$, and due to the forwarding we get $k<n-t-2\Dadv$. But what if we send 2 fragments in each message? can't we overcome this restriction somehow?}%
%\FT{Yes, there is probably a line to pursue here. There might be some link with finite projective planes (e.g. Fano's plane), as often in cases involving placement problems (which fragments should be assigned to which processes) and coding.}

We begin with a few technical lemmas.
\begin{lemma}
	\label{lemma:stored:sigs:valid}
	If a correct process $p_u$ stores signatures for some hash value $h'$, these signatures are all valid and contain a signature $\sig_s=(\SIGN_s(h'),s)$ for~$h'$ by~\psender.
\end{lemma}
\renewcommand{\lemcnt}{\ref{lemma:stored:sigs:valid}}
\begin{lemmaProof}
	As $p_u$ initially stores no signature, $p_u$ must have executed one of the \store statements for $h'$.
	As all \store operations that store signatures for some hash value $h'$ (at \cref{line:store:in:SEND,line:sign:a:hash:in:SEND,line:store:in:FORWARD,line:sign:a:hash:in:FORWARD,line:store:in:BUNDLE}) are guarded by calls to \isValid (at \cref{line:isValid:in:SEND,line:isValid:in:FORWARD,line:isValid:in:BUNDLE}). \isValid ensures that signatures received in the message that triggered this code, are all valid and contain a valid signature by $\psender$ for $h'$. Note that $p_u$ may add its own signature for~$h'$ and store it along with the other signatures. In any case, all the stored signatures are valid for~$h'$, and they contain a signature $\sig_s=(\SIGN_s(h'),s)$ for~$h'$ by~\psender.
\end{lemmaProof}


\begin{lemma}\label{lemma:stored:fragments:are:valid}
	If a correct process $p_u$ stores a message fragment and its proof of inclusion, $(\tilde m_j,\pi_j,j)$, for some hash value $h'$, then the Merkle proof of inclusion $\pi_j$ is valid with respect to~$h'$, that is $\MerkleVerify(h',\pi_j,\tilde m_j,j)=\valid$.
\end{lemma}
\renewcommand{\lemcnt}{\ref{lemma:stored:fragments:are:valid}}
\begin{lemmaProof}
	The proof is similar to that of \cref{lemma:stored:sigs:valid}. A correct process stores fragments and their proof of inclusion for a hash $h'$ at \cref{line:store:in:SEND,line:store:my:fragment:in:FORWARD,line:store:in:BUNDLE,line:store:my:fragment:in:BUNDLE}, when receiving \send, \forward, or \bundle messages, respectively. The fragments stored at these lines and their proof have been received through the corresponding message, whose content is verified by a call to \isValid (at \cref{line:isValid:in:SEND,line:isValid:in:FORWARD,line:isValid:in:BUNDLE}). \isValid (described in \cref{algo:helper:isValid}) checks that proofs of inclusion are valid for the corresponding hash.
\end{lemmaProof}

The following notion of \emph{valid} messages will be used throughout the analysis to indicate messages containing only valid information, as the algorithm dictates. In particular, 
\begin{definition}[Valid messages]\label{def:valid}
	We say that a message of type \send, \forward, or \bundle is \emph{valid} if \isValid returns $\true$ at line~\ref{line:isValid:in:SEND}, \ref{line:isValid:in:FORWARD}, or \ref{line:isValid:in:BUNDLE}, respectively, upon the \df{receipt} of that message.
\end{definition}
Operatively, valid messages satisfy the following which is immediate from the definition of the \isValid  function (\cref{algo:helper:isValid}).
\begin{corollary}\label{cor:valid}
	To be valid, a message must meet the following criteria: (i) all the signatures it contains must be valid and correspond to the hash included in the message; (ii) it must contain a signature by the designated sending process, \psender; and (iii) all Merkle inclusion proofs must be valid with respect to the hash included in the message. In addition, (iv) a \bundle message must contain more than $(n+t)/2$ signatures.
\end{corollary}

We now show that the correct parties always send valid messages. However, they might receive invalid messages sent by Byzantine nodes. 
\begin{lemma}\label{lem:all:msgs:sent:valid}
	All \send, \forward, or \bundle messages sent by a correct node~$p_u$, are valid.  
\end{lemma}
\renewcommand{\lemcnt}{\ref{lem:all:msgs:sent:valid}}
\begin{lemmaProof}
	The only correct node that sends \send messages is~$\psender$ at \cref{ln:v3.1:sendFrag}. Indeed, this message will contain a valid signature by~$\psender$ and all Merkle proofs are valid, by \cref{line:fragments:for:m,line:ps:signs:hash}.
	
	
	Now consider a \forward message sent either at lines~\ref{line:v3.1:bcast:forward} or~\ref{line:v3.1:forward:after:forward}. To reach there, $p_u$ has passed \cref{line:isValid:in:SEND} or \cref{line:isValid:in:FORWARD}, which guarantees $p_u$ received a valid signature for~$h'$ made by~$\psender$ (where $h'$ is the hash in the received message triggering this code). 
	Then in \cref{line:store:in:SEND} or in \cref{line:store:in:FORWARD}, 
	$p_u$ stores a signature of~$\psender$ for this~$h'$. Then, at \cref{line:condition:sign:hash:SEND,line:sign:a:hash:in:SEND,line:sign:a:hash:in:FORWARD}, 
	$p_u$  signs the same~$h'$. Thus, conditions (i) and (ii)  of \cref{cor:valid} hold, and if the \forward is sent at \cref{line:v3.1:forward:after:forward}, then condition (iii) vacuously holds as well.
	If the \forward message is sent at \cref{line:v3.1:forward:after:send}, it contains a Merkle proof that was stored by~$p_u$ for the same~$h'$, which by \cref{lemma:stored:fragments:are:valid} is valid; thus condition (iii) holds in this case as well.
	
	Finally, consider a \bundle message. For the transmission at \cref{line:v3.1:bundle:comm}, conditions (i) and~(ii) of \cref{cor:valid} follow from an argument similar to the one explained for \forward messages above. Condition (iii) follows since the Merkle proofs were computed at \cref{line:v3.1:recomputing:frags:with:proofs} by $p_u$ and match the same hash value~$h'$ used in that \bundle message, as enforced by \cref{line:hashes:equal:b4:delivery}. 
	For the broadcast at \cref{line:v3.1:bundle:with:bot}, conditions (i) and~(ii) follow since the signatures come from the incoming \bundle message at \cref{line:arrival:BUNDLE}. These signatures are valid and contain the signature of~$\psender$ due to the condition in \cref{line:isValid:in:BUNDLE}. Condition (iii) follows similar to the case of a \forward message.
	%
	Finally, note that in both cases there are more than $(n+t)/2$ signatures, either by \cref{line:quorum:sigs:enough:fragments} or by \cref{line:bundle:contains:quorum:BUNDLE}, respectively. This ensures condition~(iv). 
\end{lemmaProof}




%\FT{I've replaced $p_k$ with $p_u$ in the following, to avoid a conflict of notation with $\ECCthreshold$, the reconstruction threshold for the erasure code. Similarly, I've replaced $p_\ell$ with $p_x$ to avoid a conflict with $\ell$, the delivery power of the algorithm.}

%\FT{I've moved \cref{lem:single:hash:sign} down as it refers to valid messages, which have just been introduced. \cref{cor:valid,lem:all:msgs:sent:valid} do not use it.}%
\begin{lemma}\label{lem:single:hash:sign}
	A correct process $p$ signs a most a single hash value~$h$.
\end{lemma}
\renewcommand{\lemcnt}{\ref{lem:single:hash:sign}}
\begin{lemmaProof}
	$p$ signs a hash either at \cref{line:ps:signs:hash} (for \psender), \ref{line:sign:a:hash:in:SEND} or \ref{line:sign:a:hash:in:FORWARD}. We consider two cases, depending on whether $p$ is \psender or not.
	\begin{itemize}
		
		\item {\em Case 1:} Assume $p\neq\psender$. $p$ can  sign hashes only at \cref{line:sign:a:hash:in:SEND} or \ref{line:sign:a:hash:in:FORWARD}. By the conditions at \cref{line:condition:sign:hash:SEND,line:condition:sign:hash:FORWARD}, \cref{line:sign:a:hash:in:SEND,line:sign:a:hash:in:FORWARD} are executed only if either $p$ has not signed any hash yet, or has already signed the exact same hash $h'$. % By the condition at \cref{line:v3.1:test:forward:sent}, \cref{line:sign:a:hash:in:FORWARD} is executed only if no \forward message has been sent yet, which occurs at \cref{line:v3.1:bcast:forward,line:v3.1:forward:after:forward}. As a result, \cref{line:sign:a:hash:in:FORWARD} is executed at most once and only if \cref{line:sign:a:hash:in:SEND} has not been executed earlier. We conclude that $p$ signs a most one hash value. %, either at \cref{line:sign:a:hash:in:SEND} or~\ref{line:sign:a:hash:in:FORWARD}.
		
		\item {\em Case 2:} If $p=\psender$, because valid messages must contain $\psender$'s signature (due to calls to $\isValid()$ at \cref{line:isValid:in:SEND,line:isValid:in:FORWARD}), and because we have assumed that signatures cannot be forged,
		\cref{line:ps:signs:hash} is always executed before \cref{line:condition:sign:hash:SEND,line:v3.1:test:forward:sent}. By the same reasoning as Case 1, \psender therefore never signs a different hash at \cref{line:sign:a:hash:in:SEND} or \ref{line:sign:a:hash:in:FORWARD}. %, but might sign hashes at \cref{line:ps:signs:hash,line:sign:a:hash:in:FORWARD}. However, if \psender (which is assumed correct) executes \cref{line:sign:a:hash:in:FORWARD}, the call to \isValid at \cref{line:isValid:in:FORWARD} guarantees that $(h',\sigma_s,s)$ is present and valid in the set $\sigsset_j$ that is received at \cref{line:arrival:FORWARD}. As we have assumed that signatures cannot be forged, this implies that \psender has already signed the same hash $h'$ at \cref{line:ps:signs:hash}, which is executed only once when \psender is correct. As a result $\psender$ only ever signs one hash. %
		\qedhere
	\end{itemize}%
\end{lemmaProof}


We recall that the above lemmas, and as a consequence, the upcoming theorems, hold with high probability, assuming a computationally-bounded adversary that forges signatures or finds hash collisions with only negligible probability.
We can now prove the properties required for an MBRB algorithm, as depicted in \cref{def:mbrb}.
\begin{lemma}[MBRB-Validity]
	\label{thm:Validity}
	Suppose \psender is correct and a correct node, $p_i$, MBRB-delivers an {application message}, $m$. Then, node~\psender has previously MBRB-broadcast~$m$.
\end{lemma}
\renewcommand{\lemcnt}{\ref{thm:Validity}}
\begin{lemmaProof}
	%\FT{Naming: the pseudo-code uses $m_i$ at \cref{ln:MBRBdeliverMjSn} for the message that is mbrb-delivered by $p_i$, but this lemma and its proof use $m$. Change the pseudo-code to use $m$? (Or the lemma and the proof to use $m_i$.)}%
	Suppose $p_i$ MBRB-delivers $m$ at \cref{ln:MBRBdeliverMjSn}. Define $h'$ the hash value that renders true the condition at \cref{line:quorum:sigs:enough:fragments}, and $h$ the hash value that is computed at \cref{line:v3.1:recomputing:frags:with:proofs}. It holds $h'=h$ by \cref{line:hashes:equal:b4:delivery}, or otherwise $p_i$ could not have reached \cref{ln:MBRBdeliverMjSn}.
	%
	
	% Define $\sigsset_h'$ as the set of signatures stored by $p_i$ for~$h'$ when at \cref{line:quorum:sigs:enough:fragments}.
	% %By \cref{line:quorum:sigs:enough:fragments}, 
	% Since $|\sigsset_{h'}|>\frac{n+t}{2}$, and hence $\sigsset_h'\neq\emptyset$.
	Note that the set~$\sigsset_h$ at \cref{line:sigsset:h} contains at least $\frac{n+t}{2}$ signatures that $p_i$ stored for~$h'$, and in particular it contains at least one signature. Thus, by \cref{lemma:stored:sigs:valid}, $\sigsset_h$ must contain a valid signature %~$\sig_s$ 
	by \psender for~$h'$.
	%	By Line~\ref{ln:thereAreMoreThanStoredSignaturesForA}, $p_i$ also verifies $(m, j, sn)$ before delivering it (Line~\ref{ln:MBRBdeliverMjSn}).
	%
	Under the assumption that the adversary cannot forge signatures (\cref{sec:signatures}), and recalling that \psender is correct, the only way in which \psender could have signed~$h'$ is by executing \cref{line:ps:signs:hash} when MBRB-broadcasting some message $m'$ at \cref{ln:MBRBbroadcastMsn}; see also the proof of \cref{lem:single:hash:sign}.
	Furthermore, recall that the hash (the root of the Merkle Tree; \cref{sec:merkle}) is collision-resistant, meaning that except for negligible probability, the message $m'$ that \psender uses in \cref{ln:MBRBbroadcastMsn} satisfies $m'=m$, since it holds that $h'=\MerkleHash(m')=\MerkleHash(m)=h$.
	%see Eq.~\eqref{eq:MT:inclusion:collision-res}   \ran{need to formalize the properties of Merkle tree as a lemma, and use it here}
	% \ft{%
		%     By \cref{lemma:stored:fragments:are:valid}, all fragments $\tilde m_j$ selected at \cref{line:quorum:sigs:enough:fragments} are accompanied by a valid proof of inclusion $\pi_j$ with respect to~$h'$. 
		%     As we have assumed that Merkle root hash and Merkle proofs of inclusion are secure, the fragments $\tilde m_j$ selected by $p_i$ at \cref{line:quorum:sigs:enough:fragments} must belong to the fragments $\tilde m'_j$ computed by $\psender$ at \cref{line:fragments:for:m}.
		%     As \cref{line:quorum:sigs:enough:fragments} selects at least \ECCthreshold fragments, by property of the \ECC{} erasure code, \cref{line:v3.1:reconstruct:m} reconstructs the message $m'$ initially mbrb-broadcast by \psender at \cref{ln:MBRBbroadcastMsn}, hence $m'=m$. (And $h'=h$ at \cref{line:v3.1:recomputing:frags:with:proofs}.)
		% }%
\end{lemmaProof}

%Indeed, \psender will not sign a hash in \cref{line:sign:a:hash:in:SEND,line:sign:a:hash:in:FORWARD}, since the respective \isValid condition will not pass for~\psender. 
%    \ran{I suggest this shorter proof for why $m=m'$, the previous proof, based on the fragments and Lemma~4, is commented}\FT{The new proof looks good to me, and is more direct indeed.}

%\EMS{Ran, how about the following? In \cref{sec:merkle} we talk about collision-resistance and say that collisions occur with a negligible probability. Thus, for the rest of the paper, we assume that they never occur, i.e., h is always collision-free. This way, we don't have to include a discussion about probability in our algorithm and/or its proof.}
%\ran{the text above lemma4.8 says essentially the same. All statements hold with high probability and we assume bad events never happen. Yet, in the proof, we still need to mention the fact that the bad event did not happen, by assumption.}

\begin{lemma}[MBRB-No-duplication]
	\label{thm:duplication}
	A correct node~$p_i$ MBRB-delivers at most one {application message},~$m$.
\end{lemma}
\renewcommand{\lemcnt}{\ref{thm:duplication}}
\begin{lemmaProof}
	The condition at \cref{ln:bulljsnWasNotMBRBdelivered} directly implies the proof.
\end{lemmaProof}


\begin{lemma}[MBRB-No-duplicity]
	\label{thm:duplicity}
	No two different correct nodes MBRB-deliver different application messages.
\end{lemma}
\renewcommand{\lemcnt}{\ref{thm:duplicity}}
\begin{lemmaProof}
	Suppose, towards a contradiction, that $p_i$ MBRB-delivers $m$ and $p_x$ MBRB-delivers $m'\neq m$, where $p_i$ and $p_x$ are both correct nodes. Let us denote by $h$, resp. $h'$, the Merkle root hash returned by $\computeFragmentMerkleTree()$ for $m$, resp. for $m'$. As Merkle root hashes are assumed to be collision-resistant (\cref{sec:merkle}), $m\neq m'$ implies $h\neq h'$.
	
	By the condition at \cref{line:quorum:sigs:enough:fragments}, $p_i$ stores a set $Q_i$ with more that $(n+t)/2$ signatures for $h$. Similarly, $p_x$ stores a set~$Q_x$ with signatures for~$h'$. 
	%%  and $p_x$ stores each the sets $Q_i$, and respectively, $Q_x$, with more that $(n+t)/2$ signatures that they have each received for $h$ and $h'$, respectively. 
	%
	%
	We know that $|Q_i\cup Q_x|=|Q_i|+|Q_x|-|Q_i \cap Q_x|$.
	Thus, $|Q_i \cap Q_x|\geq |Q_i|+|Q_x|-n > 2 [(n+t)/2]-n=t$.
	In other words, $Q_i$ and $Q_x$ have at least one \emph{correct} node, $p_u$, in common that has signed both $h$ and $h'$. 
	\cref{lem:single:hash:sign}, and the fact that $p_u$ has signed both $h$ and $h'$ leads the proof to the needed contradiction.	Thus, $m=m'$, and the lemma holds.
\end{lemmaProof}

\begin{lemma}[MBRB-Local-delivery]
	\label{thm:Local}
	\sloppy
	Suppose \psender is correct and MBRB-broadcasts $m$.
	At least one correct node, say, $p_j$, MBRB-delivers $m$.
\end{lemma}
\renewcommand{\lemcnt}{\ref{thm:Local}}
\begin{lemmaProof}
	Let us denote by $h_m$ the Merkle root hash computed in \Cref{line:v3.1:MHash} when executing $\computeFragmentMerkleTree()$ on the input~$m$.
	%
	%\ft{Assume \psender is correct and MBRB-broadcasts $m$.} \ran{that's part of the statement.}
	The proof of the lemma will follow from 
	\crefrange{subobs:all:msgs:contain:h:sig_s}{subobs:one:correct:delivers:m} 
	%\crefrange{subobs:n:correct:sign:h':neq:h}{subobs:one:correct:delivers:m} 
	stated and proven below.
	
	%\EMS{Please remind the read what is a valid message of type X. Also, the proof statement is not clear. Either restrict the sender to be correct (as well as the predecessor sender) or say that the observation is true for all messages that are processed without having the if-statement in \cref{line:isValid:in:SEND,line:isValid:in:FORWARD,line:isValid:in:BUNDLE} hold,}\FT{I've added that \psender is assumed to be correct and to MBRB-broadcast $m$ just above. The assumption is implicit for all observations of \cref{thm:Local}. Do you think we need to add it when stating each observation?}
	
	\begin{subobservation}\label{subobs:all:msgs:contain:h:sig_s}
		%All valid \send, \forward, or \bundle messages received by some correct node $p_u$ contain~$h_m$, a valid signature $(\sigma_s,s)$ for~$h_m$, and only contain valid signatures $(h_m,\bull,\bull)$. 
		All valid \send, \forward, or \bundle messages received by some correct node $p_u$ contain~$h_m$, a signature $(\sigma_s,s)$ from~\psender, and contain only signatures that are valid for~$h_m$. 
	\end{subobservation}
	
	\renewcommand{\obscnt}{\ref{subobs:all:msgs:contain:h:sig_s}}
\sloppy\begin{obsProof}
%    \ran{proof revised, using Lemma~\ref{lem:all:msgs:sent:valid}}
%
Recall that $\psender$ MBRB-broadcasts $m$, thus we know that $\psender$ has included its own signature, $\sig_s=\big(\SIGN_s(h_m),s\big)$, when it propagates $\langle \send, h_m, (\tilde m_j, \pi_j,j), \sig_s \rangle$ (\crefrange{line:fragments:for:m}{ln:v3.1:commV1ldotsVn}).
%
Consider a correct node $p_u$ that receives a \send, \forward, or \bundle message containing a hash value $h_u$ at lines~\ref{ln:sendRx:SEND}, \ref{line:arrival:FORWARD}, or~\ref{line:arrival:BUNDLE}. 
By \cref{lem:all:msgs:sent:valid}, this message is valid, and thus, contains $\psender$'s signature on~$h_u$, and only valid signatures for~$h_u$. 
Since $\psender$ is correct, by \cref{lem:single:hash:sign} it does not sign another hash $h'\neq h_m$. 
Under the assumption that signatures cannot be forged, the above implies that $h_u=h_m$.
\end{obsProof}
	
	%   
	%
	%   
	%     \ft{Recall that in order to be valid, a message must meet the following three criteria: (i) all the signatures it contains must be valid and correspond to the hash included in the message; (ii) it must contain a signature by the designated sending process, \psender; and (iii) all Merkle inclusion proofs must be valid. In addition, a \bundle message must contain more than $(n+t)/2$ signatures.}\ran{why does the fact on bundle matter here?}
	%     Since $\psender$ MBRB-broadcasts $m$, we know that $\psender$ has included its own signature, $\sig_s=\big(\SIGN_s(h_m),s\big)$, when it propagates $\langle \send, h_m, (\tilde m_j, \pi_j), \sig_s \rangle$ (\crefrange{line:fragments:for:m}{ln:v3.1:commV1ldotsVn}).
	% 	Since $\psender$ is correct, by \cref{lem:single:hash:sign} it does not sign another hash $h'\neq h_m$.
	%
	%   Consider a correct node $p_u$ that receives a \send, \forward, or \bundle message containing a hash value $h_u$ at lines~\ref{ln:sendRx:SEND}, \ref{line:arrival:FORWARD}, or~\ref{line:arrival:BUNDLE}. All three message handlers are guarded by the helper function $\isValid$ (at \cref{line:isValid:in:SEND,line:isValid:in:FORWARD,line:isValid:in:BUNDLE}).
	% By \cref{line:isValid:sigs:contain:ps:sign}, \isValid{} verifies that some $(\sigma_s,s)$ is present in the set of signatures received by~$p_u$, and that it is valid for~$h_u$. As we have assumed that signatures cannot be forged, the fact that \psender only ever signs $h_m$ implies $h_u=h_m$. By \cref{line:isValid:sigs:are:valid}, \isValid also ensures that all received signatures are valid and correspond to $h_m$.
	
	\begin{subobservation}\label{subobs:n:correct:sign:h':neq:h}
		A correct party~$p_u$ signs and stores only values that correspond to~$h_m$. All these signatures are valid.%
	\end{subobservation}
	
	%\FT{Changing the word order to avoid the ambiguity re. the distribution of `only' onto either `for~$h_m$' (what we intend), or onto `valid' (which could be understood in the previous version.)}%
	%\ran{"sign signatures"?  Usually "only" comes right before the phrase it modifies. If a party  signs $h_m$ and no other value, the modified part is $h_m$, and the sentence  should read ``signs only the value~$h_m$''. I would change to ``signs and stores only values that correspond to~$h_m$''}%
	%\FT{+1. I've changed it accordingly.}
	%\FT{Enriching the lemma somewhat as useful later on.}
	%
	% There is no correct $p_u$ that signs or stores a valid signature for $h'$, when $h'\neq h_m$.
	%\EMS{The proof is missing to mention the tests whether such storing had occurred before, see lines 15, 23, 26, and 30}\FT{The proof states that if a correct process signs or stores a valid signature for some hash $h'$, then this signature is in fact for $h'=h_m$ (maybe it should be rephrased that way), so the focus is not on whether signing or storing does occur (and on the tests that limit their occurrence), but on what we can say when they do occur. That is the reason why the proof of \cref{subobs:n:correct:sign:h':neq:h} does not mention the test at lines 15, 23, 26, and 30. Does this make it clearer?}\ran{looks good to me, I slightly changed the statement to indicate that $p$ can't store invalid signatures as well.}
	\renewcommand{\obscnt}{\ref{subobs:n:correct:sign:h':neq:h}}
	\begin{obsProof}
		If $p_u=\psender$, it MBRB-broadcasts a single message and executes \cref{line:ps:signs:hash} only once, signing $h_m$.
		Besides \cref{line:ps:signs:hash}, a correct process $p_u$ only signs or stores signatures after receiving a valid \send, \forward, or \bundle message (at \cref{line:store:in:SEND,line:sign:a:hash:in:SEND,line:store:in:FORWARD,line:sign:a:hash:in:FORWARD,line:store:in:BUNDLE}), and when it does, $p_u$ only ever signs the hash received in the message, and only stores signatures received in the message, or the signature it has just signed. By \cref{subobs:all:msgs:contain:h:sig_s}, this implies $p_u$ never signs any $h'\neq h_m$. Further, it only stores \emph{valid} signatures (since the receives message is valid) and only for~$h_m$, by \cref{lemma:stored:fragments:are:valid,subobs:all:msgs:contain:h:sig_s}.
	\end{obsProof}
	
	%\EMS{Do you mean to say '$p_u$'s valid signature of $h_m$'? The same fo Observation 9.4.}\FT{Yes indeed. I've added `valid' to remove any ambiguity.}
	
	\begin{subobservation}\label{subobs:all:correct:send:forward:form}
		If a correct process $p_u$ broadcasts a \forward message, this message is of the form $\langle \forward, h_m, \bull, \{\sig_s,\sig_u\} \rangle$, where $\sig_s,\sig_u$ are $\psender$'s and $p_u$'s   valid signatures for~$h_m$. 
	\end{subobservation}
	
	%%Additionally, if $\frag\ne \bot$, then it is valid for~$h_m$.
	%
	%%%OLD:
	%If a correct process $p_u$ broadcasts a \forward message, this message is of the form $\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$, where $\sig_u=(\SIGN_u(h_m),u)$ is $p_u$'s \ft{valid} signature of $h_m$,  and $\bullet$ represents any sequence of values. 
	
	\renewcommand{\obscnt}{\ref{subobs:all:correct:send:forward:form}}
	\begin{obsProof}
		Consider a correct process $p_u$ that broadcasts a message $\langle \forward,\allowbreak h',\bull,\sigsset \rangle$ either at lines~\ref{line:v3.1:bcast:forward} or~\ref{line:v3.1:forward:after:forward}.
		By \cref{subobs:all:msgs:contain:h:sig_s}, $h'=h_m$.
		The observation then follows from \cref{lem:all:msgs:sent:valid}.
		%\FT{I've simplified the proof: since \forward messages only include 2 signatures now, I believe just referring to \cref{lem:all:msgs:sent:valid} (all messages sent by correct processes are valid) is enough once we have $h'=h_m$.}
	\end{obsProof}
	%, and $\sigsset$ only contain signatures that are valid for~$h'=h_m$. 
	% % Francois: Earlier version, commented out
	% Since the sent message must be valid (\cref{lem:all:msgs:sent:valid}), it must contain $\psender$'s valid signatures for~$h_m$, \ie $\sig_s\in\sigsset$.
	% %
	% Finally, due to \cref{line:sign:a:hash:in:SEND,line:sign:a:hash:in:FORWARD}, 
	% before $p_u$~broadcasts a \forward message, it signs the hash value contained in that message, which by the above is~$h_m$. This signature is sent in the \forward message, completing the proof of the observation.
	% %
	%
	%
	% By \cref{line:condition:sign:hash:SEND,line:sign:a:hash:in:SEND,line:sign:a:hash:in:FORWARD}, 
	% When $p_u$ broadcasts $\langle \forward, h_m, \bull, \bull \rangle$ at lines~\ref{line:v3.1:bcast:forward} or~\ref{line:v3.1:forward:after:forward}, it has signed some message hash $h_u$. By \cref{subobs:n:correct:sign:h':neq:h}, $h_u=h_m$. By \cref{subobs:all:msgs:contain:h:sig_s} when $p_u$ executes lines~\ref{line:v3.1:bcast:forward} or~\ref{line:v3.1:forward:after:forward}, it must have stored $\sig_s=(\SIGN_s(h_m),s)$ at lines~\ref{line:store:in:SEND} or \ref{line:store:in:FORWARD}, respectively. As a result, any message broadcast by $p_u$ is of the form $\langle \forward, h_m, \bull, \{\sig_s,\sig_u \} \rangle$, 
	% %%where $\sigsset$ contains at least 
	% with $\sig_u=(\SIGN_u(h_m),u)$ and $\sig_s=(\SIGN_s(h_m),s)$, \ie $p_u$ and~\psender's valid signatures for~$h_m$. %%Finally, note that $\sigsset$ contains only signatures that were stored by~$p_u$. By \cref{subobs:n:correct:sign:h':neq:h} all these signatures are valid for~$h_m$.
	%
	% Finally, consider the case where $\frag=(\tilde m_u,\pi_u)$. This means that $p_u$ broadcast this \forward at  \cref{line:v3.1:forward:after:send}, since otherwise $\frag=\bot$. Then, note that due to \cref{line:isValid:in:SEND}, we have that $\MerkleProof(h_m,\pi_u,\tilde m_u)=\true$. Thus, this message fragment and Merkle proof is valid for~$h_m$.
	
	%\newcommand{\frwdReceiveSet}{F_{\uparrow}}
	\newcommand{\frwdReceiveSet}{F_{\mathsf{recv}}}
	
	We now define $\frwdReceiveSet$ to be the set of correct nodes that receive a valid message $\langle \forward,\allowbreak h_m,  \bull, \sigsset \rangle$ at \cref{line:arrival:FORWARD}, where $\sigsset$ contains $\psender$'s valid signature for~$h_m$. We analyze its size and the behavior of such nodes in the following observations.
	
	%\FT{Adding the extra observation to show that $\frwdReceiveSet\neq\emptyset$. We need it to apply the pigeonhole principles (where we divide by $|\frwdReceiveSet|$). The proof is a bit verbose: it can maybe be streamlined.}
	\begin{subobservation}\label{subobs:frwdReceiveSet:not:empty}
		% If \psender is correct and MBRB-broadcasts $m$, then 
		$\frwdReceiveSet$ contains at least one correct process, i.e. $\frwdReceiveSet\neq\emptyset$.
	\end{subobservation}
	\renewcommand{\obscnt}{\ref{subobs:frwdReceiveSet:not:empty}}
	\begin{obsProof}
		If \psender is correct and MBRB-broadcasts $m$, it executes \cref{ln:v3.1:commV1ldotsVn} and disseminates messages of the form $\langle \send, h_m, (\tilde m_j, \pi_j), \sig_s \rangle$ to all processes, where $\sig_s$ is \psender's signature of $h_m$. By definition of the message adversary, these \send messages are received by at least $c-d$ correct processes. 
		
		By Assumption~\ref{asm:MBRBassumptionR}, $n>3t + 2{\Dadv}$, and therefore $c-d\geq n-t-d > 0$. At least one correct process $p_x$, therefore, receives one of the \send messages disseminated by \psender at \cref{ln:v3.1:commV1ldotsVn}. By \cref{subobs:all:msgs:contain:h:sig_s}, this message is valid, and handled by $p_x$ at \crefrange{ln:sendRx:SEND}{line:v3.1:forward:after:send}. 
		
		By \cref{subobs:n:correct:sign:h':neq:h}, $p_x$ only signs signatures for $h_m$, and thus passes the test at \cref{line:condition:sign:hash:SEND}, and reaches \cref{line:v3.1:forward:after:send}, where it disseminates a \forward message. By \cref{subobs:all:correct:send:forward:form}, this message is of the form $\langle \forward, h_m, \bull, \{ \sig_s,\sig_x \} \rangle$, and is valid. As above, by definition of the message adversary, this \forward message is received by at least $c-d>0$ correct processes. By definition these processes belong to $\frwdReceiveSet$, which yield $|\frwdReceiveSet|>0$ and $\frwdReceiveSet\neq\emptyset$.
	\end{obsProof}
	
	\begin{subobservation}\label{subobs:all:correct:rv:FW:do:send:FW}
		Any $p_u \in \frwdReceiveSet$ broadcasts a \forward message 
		$\langle \forward,\allowbreak h_m,  \bull,$ $\{\sig_s,\sig_u\} \rangle$, where $\sig_s $ and $\sig_u$ are $\psender$ and $p_u$'s valid signatures for~$h_m$, respectively.
	\end{subobservation}
	
	%$\langle \forward,\allowbreak h_m,  \bull, \sigsset' \rangle$,
	%that also contains 
	
	%  \FT{Adapting the observation's statement to match the new pseudo-code.}%
	%Let $\frwdReceiveSet$ be the set of correct nodes that receive a valid message $\langle \forward,$ $h_m,$ $ \bull, \{\sig_s, \bullet\} \rangle$ at \cref{line:arrival:FORWARD}, where $\bullet$ represents any sequence of values. {Any} such~$p_u \in \frwdReceiveSet$ broadcasts a message $\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$, where $\sig_u=$ $\big(\SIGN_u(h_m),$ $u\big)$ is $p_u$'s \ft{valid} signature of $h_m$.
	
	\renewcommand{\obscnt}{\ref{subobs:all:correct:rv:FW:do:send:FW}}
	\begin{obsProof}
		Let $p_u\in \frwdReceiveSet$ upon receiving a valid \forward message $\langle \forward,\allowbreak h_m,  \bull, \sigsset \rangle$ at \cref{line:arrival:FORWARD}. 
		By the condition of \cref{line:v3.1:test:forward:sent}, $p_u$ has either previously sent a \forward message at \cref{line:v3.1:bcast:forward} or it will send such a message at~\cref{line:v3.1:forward:after:forward}. 
		In both cases, \cref{subobs:all:correct:send:forward:form} applies and guarantees that this message contains $h_m$ and both $p_u$'s and $\psender$'s valid signatures.
		%any node $p_u$ in $\frwdReceiveSet$ sends at least one message $\langle \forward, h', \bull, \bull\rangle$ either at lines~\ref{line:v3.1:bcast:forward} or~\ref{line:v3.1:forward:after:forward}. \cref{subobs:all:correct:send:forward:form} applies and concludes the proof.
	\end{obsProof}
	
	{Note that $\frwdReceiveSet$ is defined over an entire execution of \cref{alg:3.1:merkle:trees}. \cref{subobs:all:correct:rv:FW:do:send:FW} therefore states that any correct process $p_u$ that receives a valid \forward message \emph{at some point of its execution} also broadcasts a matching \forward message \emph{at some point of its execution}. \df{The two} events (receiving and sending a \forward message) might, however, occur in any order. For instance, $p_u$ might first receive a \send message from \psender at \cref{ln:sendRx:SEND}, disseminate a \forward message as a result at \cref{line:v3.1:forward:after:send}, and later on possibly receive a \forward message from some other process at \cref{line:arrival:FORWARD}. Alternatively, $p_u$ might first receive a \forward message at \cref{line:arrival:FORWARD}, and disseminate its own \forward message at \cref{line:v3.1:forward:after:forward} as a result. In this second case, $p_u$ might also eventually receive a \send message from \psender (at \cref{ln:sendRx:SEND}). If this happens, $p_u$ will disseminate a second \forward message at \cref{line:v3.1:forward:after:send}. A correct process, however, never disseminates more than two \forward messages (at \cref{line:v3.1:forward:after:send,line:v3.1:forward:after:forward}).}
	
	\begin{subobservation}\label{subobs:all:forwd:hm:received:by:Fdown}
		Any broadcast of 
		% $\langle \forward, h_m, \frag, \sigsset \rangle$ 
		$\langle \forward, h_m, \frag, \{ \sig_s,\sig_u \} \rangle$
		%$\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$ 
		by a correct $p_u \in \frwdReceiveSet$ arrives to at least $c-\Dadv$ correct nodes that are each, eventually, in $\frwdReceiveSet$.
	\end{subobservation}
	
	%\FT{Adapting format of \forward message to match the new pseudo-code.}
	
	\renewcommand{\obscnt}{\ref{subobs:all:forwd:hm:received:by:Fdown}}
	\begin{obsProof}
		Each broadcast by a correct $p_u$ of a \forward message
		is eventually received by at least $c-\Dadv$ correct nodes by definition of the message adversary.
		By \cref{subobs:all:correct:send:forward:form} the \forward message contains~$h_m$, by \cref{lem:all:msgs:sent:valid} it is valid. Thus, each of its at least $c-\Dadv$ correct recipients belong in $\frwdReceiveSet$, by definition.
		%
		%
		%
		% Each broadcast by a correct $p_u$ of 
		%    a \forward message
		%    %$\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$ 
		%    is eventually received by at least $c-\Dadv$ correct nodes by definition of the message adversary.
		%    By \cref{subobs:all:correct:send:forward:form} the \forward message contains $h_m$, $\psender$'s signature, and only valid signatures for~$h_m$. AdditioLnally, either $\frag$ is $\bot$ or is a valid message fragement and Merkle proof for~$h_m$.
		%    Therefore, this message will be considered valid by its recipient. 
		%    Hence, all the correct recipients of this message belong to~$\frwdReceiveSet$, by definition.
	\end{obsProof}
	%\EMS{How about using 'chain reaction' instead of 'chains'. We don't want the reader to start asking for the definition of chairs and wonder what we mean. But, 'chain reaction' is more intuitive. Then you can also replace chaining with 'this process of chain reaction'}\FT{Yes, I agree. I've changed the text accordingly.}
	
	{Because \forward messages are disseminated at \cref{line:v3.1:forward:after:forward}, the reception and sending of \forward messages by correct processes will induce a `chain reaction' until a correct process is reached that has already disseminated a \forward message. This `chain reaction' mechanism is the intuitive reason why some correct process will eventually receive enough distinct \forward messages to trigger an MBRB-delivery, as captured by the following observation.}
	
	\begin{subobservation}\label{subobs:exist:correct:c-d:sigs}
		There exists a correct node~$p_j$ that receives messages 
		%$\langle \forward, h_m,$ $\bull,$ $\{\sig_u,$ $\sig_s,$ $\bullet \} \rangle$ 
		$\langle \forward, h_m,\bull, \allowbreak\sigsset_u=\allowbreak\{\sig_s,\allowbreak\sig_u\} \rangle$
		from at least $(c-\Dadv)$ distinct correct nodes $p_u$, 
		where $\sig_s=(\SIGN_s(h_m),s) $ and $\sig_u=(\SIGN_u(h_m),u)$ are $\psender$ and $p_u$'s valid signatures for~$h_m$, respectively,
		%where $\sigsset_u$ contains $p_u$'s valid signature for~$h_m$, $\sig_u=(\SIGN_u(h_m),u)$, 
		and the \forward message is the \emph{last} message sent by $p_u$.
	\end{subobservation}
	
	\newcommand{\frwdBcastSet}{F_{\downarrow}}
	
	\renewcommand{\obscnt}{\ref{subobs:exist:correct:c-d:sigs}}
	\begin{obsProof}
		By \cref{subobs:all:correct:rv:FW:do:send:FW}, any processes $p_u\in \frwdReceiveSet$ broadcasts at least one message $\langle \forward, h_m, \bull, \sigsset_u=\allowbreak\{\sig_s,\allowbreak\sig_u\} \rangle$, that includes $p_u$'s valid signature for~$h_m$, $\sig_u=$ $\big(\SIGN_u(h_m),u\big)$.
		%
		Consider all the \forward messages 
		%$\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$ 
		sent by nodes in $\frwdReceiveSet$ during the \emph{last time} they perform such a broadcast. 
		%
		By \cref{subobs:all:forwd:hm:received:by:Fdown}, there are $|\frwdReceiveSet|$ senders, $p_u \in \frwdReceiveSet$, such that each of $p_u$'s last broadcast of 
		%$\langle \forward, h_m, \bull, \{\sig_u, \sig_s, \bullet \} \rangle$ 
		a \forward message
		is guaranteed to be delivered to at least $c-\Dadv$ correct nodes~$p_x$, such that eventually $p_x \in \frwdReceiveSet$.
		Thus, at least $|\frwdReceiveSet|(c-\Dadv)$ such messages are received by nodes in~$\frwdReceiveSet$, overall. 
		%
		By \cref{subobs:frwdReceiveSet:not:empty}, $\frwdReceiveSet$ contains at least one process. We can, therefore, apply the pigeonhole principle, where $\frwdReceiveSet$ are the holes and the above $|\frwdReceiveSet|(c-\Dadv)$ messages are the pigeons, and observe that there exists a node~$p_j\in \frwdReceiveSet$ that will receive at least $|\frwdReceiveSet|(c-\Dadv)/|\frwdReceiveSet|$ such messages. 
		Since we limit the discussion to a \emph{single}, \ie the last, broadcast performed by each node in $\frwdReceiveSet$, 
		no node in~$\frwdReceiveSet$ receives two of the above messages that were originated by the same node in~$\frwdReceiveSet$.
		Therefore, we deduce that $p_j$ has received messages of the form $\langle \forward, h_m, \bull, \sigsset_u \rangle$ from at least $(c-\Dadv)$ \emph{distinct} correct nodes $p_u$ and the \forward message is the \emph{last} message sent by $p_u$.
	\end{obsProof}
	
	\begin{subobservation}\label{subobs:one:correct:delivers:m}
		At least one correct node MBRB-delivers $m$ from $\psender$.
	\end{subobservation}
	
	\renewcommand{\obscnt}{\ref{subobs:one:correct:delivers:m}}
	\begin{obsProof}
		By \cref{subobs:exist:correct:c-d:sigs}, there is a correct node~$p_j$ that receives messages of the form $\langle \forward, h_m, \bull, \sigsset_u \rangle$ from at least $(c-\Dadv)$ distinct correct nodes $p_u$, such that these \forward messages are the \emph{last} message sent by each $p_u$. Let us denote by $U$ the set of such processes~$p_u$, hence,  $|U|\ge c-\Dadv$.
		
		Still by \cref{subobs:exist:correct:c-d:sigs}, $p_j$ receives a valid signature $\sig_u=(\SIGN_u(h_m),u)$ from each process $p_u\in U$. It thus receives at least $(c-\Dadv)$ \emph{distinct} signatures for~$h_m$.
		The coded-MBRB-assumption (Assumption~\ref{asm:MBRBassumptionR}) says $3t + 2{\Dadv} < n$, and thus, $n + 3t + 2{\Dadv} < 2n$ and $n + t < 2n - 2t - 2{\Dadv}$.
		Since $n - t \leq c$, we have $(n+t)/ 2 < n - t - {\Dadv} \leq c - {\Dadv}$. 
		Thus, $p_j$ receives more than $(n+t )/2 $ valid distinct signatures, 
		%$\sig_u$ 
		for~$h_m$.
		
		Let us now consider the set of correct processes $S$ that receive the initial \send messages disseminated by $\psender$ at \cref{ln:v3.1:commV1ldotsVn}. Any process $p_x\in S$ receives through the \send message its allocated fragment $(\tilde m_x, \pi_x,x)$ from~\psender. By definition of the message adversary, the \send messages disseminated at \cref{ln:v3.1:commV1ldotsVn} are received by at least $c - {\Dadv}$ correct processes, therefore $|S|\geq c - {\Dadv}$. Furthermore, all processes in $S$ broadcast a \forward message at \cref{line:v3.1:forward:after:send}, and this will be their \emph{last} \forward message, due to the condition of~\cref{line:v3.1:test:forward:sent}. 
		%  By \cref{subobs:all:correct:send:forward:form} 
		By the above reasoning, this \forward message will contain their message fragment, that is, it will be of the form $\langle \forward, h_m, (\tilde m_x, \pi_x,x), \sigsset_u \rangle$. 
		By \cref{lem:all:msgs:sent:valid}, they are all valid.
		% Note that by \cref{subobs:all:correct:send:forward:form}
		% \ran{used to be \cref{lemma:stored:fragments:are:valid}, is it stil needed?} the message fragment and Merkle proof included in this message must be valid.
		
		% \ran{All comments were answered so I removed them}
		% \EMS{Justify the next sentence. Maybe by definition of S and U?}\FT{Indeed. I've done as suggested.}
		
		%\EMS{Please consider writing 'broadcast by processes in $S\cap U$ are received by $p_j$ ' instead of 'broadcast by processes in $|S\cap U|$ are received by $p_j$ '}\FT{Indeed, that was a typo, now corrected.}
		
		%\EMS{Please justify 'with their Merkle proof of inclusion $(\tilde m_x, \pi_x,x)$.'}\ft{I've referred to \cref{lemma:stored:fragments:are:valid}. Is it clearer?}\ran{revised a bit. Above the statement regarding FORWARD sent by $S$ is clear and includes justification to the Merkle proof part and its validity}
		
		By definition of $S$ and $U$, both these sets  contain only correct processes, 
		%of which there are $c$.
		thus, $|S \cup U| \le c$.
		As a result, $|S\cap U|=|S| + |U| - |S\cup U|\geq 2\times (c-\Dadv) -c = c -2\Dadv$. 
		The last \forward messages broadcast by processes in $S\cap U$ are received by $p_j$ by the definition of $U$. 
		As argued above about nodes in~$S$ (and thus applying to nodes in $S\cap U$), \forward
		messages sent by a process in $S\cap U$  contain their valid message fragment and Merkle proof of inclusion~$(\tilde m_x, \pi_x,x)$. 
		It follows that $p_j$ accumulates at least $c -2\Dadv$ distinct such message fragments with their (valid) Merkle proof of inclusion.  By \cref{asm:MBRBassumptionR}, $c -2\Dadv\geq \ECCthreshold$.
		
		%\EMS{Please justify '    The condition at \cref{line:quorum:sigs:enough:fragments} therefore eventually becomes \true for $p_j$.'. Please remind the reader why the first two conditions hold. If needed, break Observation 9.7 into several parts. }\ft{Is this clearer?}
		
		To conclude the proof, note that we have shown that $p_j$ eventually receives more than $(n+t )/2 $ valid distinct signatures for~$h_m$, and additionally, that $p_j$ accumulates at least $k$ valid message fragments with their Merkle proof of inclusion. At this point, the condition of \cref{line:quorum:sigs:enough:fragments}  becomes \true for~$p_j$.
		%
		Because the Merkle tree is fragments collision-resistant (section~\ref{sec:merkle}), once $h_m$ is fixed, 
		%Since generating a valid Merkle proof for an incorrect fragment cannot happen under our security assumption, 
		we can assume that, except with negligible probability, all the message fragments that $p_j$ has received correspond to the fragments computed by \psender at \cref{line:fragments:for:m}.
		%As we have assumed that the Merkle proofs of inclusion $\pi_x$ are secure, the received fragments $\tilde m_x$ all belong to the set of fragments computed by \psender at \cref{line:fragments:for:m}. 
		By the parameters of the ECC, we use %(\cref{sec:ECC-instantiation}) 
		it can recover the message $m$ from any $\ECCthreshold$ or more (correct) fragments generated by~$\psender$, where missing fragments are considered as erasures. Therefore,
		the message $m_j$ reconstructed at \cref{line:v3.1:reconstruct:m} by $p_j$ is the message initially MBRB-broadcast by $\psender$. As a result $m_j=m$, and 
		%by \cref{subobs:all:msgs:contain:h:sig_s} \ran{why is this observation relevant here?}
		$p_j$ MBRB-delivers~$m$ at \cref{ln:MBRBdeliverMjSn}.
	\end{obsProof}
	
\end{lemmaProof}

\cref{thm:Global} is the detailed version of \cref{thm:SGlobal}.

\begin{lemma}[MBRB-Global-delivery]
	\label{thm:Global}
	Suppose a correct node, $p_i$, MBRB-delivers an {application message}~$m$.
	%At least $\ell=\displaystyle c\left(1-\frac{\Dadv}{c-\ECCthreshold+1}\right)$ correct nodes MBRB-deliver $m$.
	{At least $\ell=\displaystyle c - \Dadv\left(\frac{1}{1-\left(\frac{\ECCthreshold-1}{c-\Dadv}\right)}\right)$ correct nodes MBRB-deliver~$m$.}
\end{lemma}
\renewcommand{\lemcnt}{\ref{thm:Global}}
\begin{lemmaProof}
	%  \newcommand{\bundleReceiveSet}{\ensuremath{B_{\uparrow}}\xspace}
	%  \newcommand{\bundleKReceiveSet}{\ensuremath{B_{\ECCthreshold\uparrow}}\xspace}
	%  \newcommand{\bundleSendSet}{\ensuremath{B_{\downarrow}}\xspace}
	%  
	Suppose a correct node $p_i$ MBRB-delivers $m$ (\cref{ln:MBRBdeliverMjSn}). Let us denote by $h_m$ the Merkle root hash returned by $\computeFragmentMerkleTree()$ for $m$.
	%
	%In the following, a \bundle message for a hash value $h'$ received by a correct process is said to be \emph{valid} if it passes the two conditions at \cref{line:isValid:in:BUNDLE,line:bundle:contains:quorum:BUNDLE}, i.e. its signatures and proofs are valid, it contains a signature $(\SIGN_s(h'),s)$ from~\psender, and it contains 
	%  %a Byzantine quorum of signatures for $h'$\ft{, i.e. it contains 
		%  more than $(n+t)/2$ distinct signatures for~$h'$. 
		%%\ran{No need, this is already defined in \cref{def:valid}}
		%  
		The proof follows a counting argument on the \bundle messages disseminated by correct processes at \cref{line:v3.1:bundle:comm,line:v3.1:bundle:with:bot}. In the following, if a correct process disseminates a \bundle message both at \cref{line:v3.1:bundle:comm,line:v3.1:bundle:with:bot}, we only consider the one from \cref{line:v3.1:bundle:comm}.
		
		
		\begin{subobservation}\label{subobs:all:bundle:valid:hm}
			All valid \bundle messages exchanged during the execution of \cref{alg:3.1:merkle:trees} contain~$h_m$, the Merkle root hash of the message~$m$, where $m$ is the message MBRB-delivered by~$p_i$.
		\end{subobservation}
		%    \EMS{It took me forever to read the statement below.}
		%\EMS{Is it ok to rephrase the statement to the following?     'Let $\langle \bundle, h_m \rangle$ be a valid implementation message for which the correct node $p_i$ MBRB-delivers the application message~$m$.     It holds that $h_m$ is the Merkle root hash of the message~$m$'}\FT{$h_m$ has already been defined above (at the start of the proof of the Lemma) as the hash of $m$, so the fact that  $h_m$ is $m$'s hash cannot be the conclusion of this observation. Maybe the confusion/difficulty is due to different ways of interpreting (sub)Observation: \cref{subobs:all:bundle:valid:hm} is embedded in the proof of \cref{thm:Global}, so any assumption/notation/variable/results already defined/shown in the proof of the lemma is assumed to hold within the proof of the observation as well. I've added `exchanged during the execution of \cref{alg:3.1:merkle:trees}' in the statement of \cref{subobs:all:bundle:valid:hm} in an attempt to make the origin of the \bundle messages clearer.}
		
		\renewcommand{\obscnt}{\ref{subobs:all:bundle:valid:hm}}
		\sloppy\begin{obsProof}
			%A correct process may send \bundle messages either at line~\ref{line:v3.1:bundle:comm} or~\ref{line:v3.1:bundle:with:bot}.
			% \begin{itemize}
				% \item At \cref{line:v3.1:bundle:comm}, $h$, $(\tilde m'_i,\pi'_i)$, and $(\tilde m'_j,\pi'_j)$ are constructed at \cref{line:v3.1:recomputing:frags:with:proofs}. The fragments $(\tilde m'_i,\pi'_i)$, and $(\tilde m'_j,\pi'_j)$ are therefore valid by construction. By \cref{lemma:stored:sigs:valid}, the sets $\sigsset_h$ that is extracted at \cref{line:sigsset:h} only contains valid signatures, and \psender's signature for $h$. Finally, due to the condition at \cref{line:quorum:sigs:enough:fragments}, $\sigsset_h$ contains strictly more than $\frac{n+t}{2}$ signatures. The \bundle message is therefore valid.
				% \item At \cref{line:v3.1:bundle:with:bot}, $h'$, $(\tilde m'_i,\pi'_i)$, and $\sigsset$ have been obtained from the \bundle message received at \cref{line:arrival:BUNDLE}. Due to the tests performed at \cref{line:isValid:in:BUNDLE,line:bundle:contains:quorum:BUNDLE}, the \bundle message sent at \cref{line:v3.1:bundle:with:bot} is also valid.
				% \end{itemize}
			Consider a valid message $\langle \bundle,\allowbreak h', \frag'_j,\allowbreak \frag'_i, \sigsset' \rangle$. By definition of a valid \bundle message, $\sigsset'$ contains only valid signatures for $h'$ and $|\sigsset'|>(n+t)/2$. Let us denote by $\sigsset_m$ the set of signatures for $h_m$ stored by $p_i$ when $p_i$ MBRB-delivers $m$ at \cref{ln:MBRBdeliverMjSn}. By the condition at \cref{line:quorum:sigs:enough:fragments}, $|\sigsset_m|>(n+t)/2$. By a reasoning identical to that of \cref{thm:duplicity}, these two inequalities imply that $\sigsset'\cap \sigsset_m$ contains the signatures from at least one common correct process, $p_u$. As signatures cannot be forged, $p_u$ has issued signatures for both $h'$ and $h_m$, and by \cref{lem:single:hash:sign}, $h'=h_m$. 
			To complete the proof, note that by the definition of a valid message, the signatures it contains are valid with respect to the hash value it carries. Hence, all valid \bundle messages must contain the hash value~$h_m$ of the application message~$m$ that matches the signatures $\sigsset'$ they contain. 
			%To complete the proof for sent messages,  recall that \cref{lem:all:msgs:sent:valid} guarantees that correct processes only send valid \bundle messages, hence the same argument applies here as well.
		\end{obsProof}
		
		Let \bundleSendSet be the set of correct nodes that disseminate at least one \bundle message during their execution. Similarly, let \bundleReceiveSet be the set of correct nodes that receive at least one valid \bundle message from a correct node during their execution. The following holds.
		%Since $p_i$ MBRB-delivers $m$ at \cref{ln:MBRBdeliverMjSn},  it must have disseminated \bundle messages at \cref{line:v3.1:bundle:comm}. This implies that $p_i\in\bundleSendSet$ and $\bundleSendSet\neq\emptyset$.
		%The \bundle messages sent by~$p_i$ eventually reach at least $c-\Dadv>0$ correct processors, hence, $\bundleReceiveSet\neq\emptyset$.
		%%  Similarly, by definition of the network adversary, at least $c-\Dadv>0$ correct processes must receive the \bundle messages sent at \cref{line:v3.1:bundle:comm} by $p_i$, implying $\bundleReceiveSet\neq\emptyset$.
		
		%% \FT{The following is incorrect, removing}
		% \begin{subobservation}\label{subobs:bundleR:implies:bundleS}
			%   $|\bundleReceiveSet|\leq|\bundleSendSet|$
			% \end{subobservation}
		
		% \renewcommand{\obscnt}{\ref{subobs:bundleR:implies:bundleS}}
		% \begin{obsProof}    
			%   Let $p_u\in\bundleReceiveSet$. $p_u$ executes \cref{line:arrival:BUNDLE,line:isValid:in:BUNDLE}, reaches \cref{line:test:if:already:bundle}, and disseminates a (valid) \bundle message at \cref{line:v3.1:bundle:with:bot} if it has not done so already. Therefore, $p_u\in\bundleSendSet$, which yields $\bundleReceiveSet \subseteq \bundleSendSet$ and implies the observation's inequality.
			% \end{obsProof}

  		
		\medskip
		\cref{subobs:bundleR:and:bundleS:geq:c-d} is a detailed version of~\cref{subobs:SbundleR:and:bundleS:geq:c-d} in \cref{thm:SGlobal}.
		
		\begin{subobservation}\label{subobs:bundleR:and:bundleS:geq:c-d}
			$c \geq |\bundleReceiveSet| \geq c-\Dadv$ and $c \geq |\bundleSendSet| \geq c-\Dadv$.
		\end{subobservation}
		
		\renewcommand{\obscnt}{\ref{subobs:bundleR:and:bundleS:geq:c-d}}
		\begin{obsProof}
			Since \bundleSendSet and \bundleReceiveSet contain only correct processes, trivially $c \geq |\bundleSendSet|$ and $c \geq |\bundleReceiveSet|$.
			Since $p_i$ MBRB-delivers $m$ at \cref{ln:MBRBdeliverMjSn},  it must have disseminated \bundle messages of the form $\langle \bundle, h_m, (\tilde m'_i,\pi'_i), (\tilde m'_j,\pi'_j), \sigsset_h \rangle$ at \cref{line:v3.1:bundle:comm}. %This implies that $p_i\in\bundleSendSet$ and $\bundleSendSet\neq\emptyset$.
			The \bundle messages sent by~$p_i$ eventually reach at least $c-\Dadv$ correct processors, as the message adversary can remove at most~$\Dadv$ of these \bundle messages. % we had `omit' instead of remove.
			By \cref{lem:all:msgs:sent:valid}, %\cref{subobs:all:bundle:valid:hm}, 
			these \bundle messages are valid. 
			Hence, $\bundleReceiveSet\ge c-\Dadv>0$ proves the lemma's first part. 
			
			%  By \cref{line:v3.1:bundle:comm}, $p_i$ has disseminated messages of the form $\langle \bundle, h_m, (\tilde m'_i,\pi'_i), (\tilde m'_j,\pi'_j), \sigsset_h \rangle$ to all processes, where $(\tilde m'_j,\pi'_j)_j$ are the fragments and Merkle proofs of inclusion reconstructed from $m$ by $p_i$ at \cref{line:v3.1:recomputing:frags:with:proofs}. By \cref{lemma:stored:sigs:valid} all these messages are valid. By definition of the message adversary at least $c- {\Dadv}$ correct processes eventually receive these messages, which implies $|\bundleReceiveSet| \geq c-\Dadv$ and proves the first part of the lemma.  
			
			The processes in $\bundleReceiveSet$ (which are correct) execute \cref{line:arrival:BUNDLE,line:isValid:in:BUNDLE}, and reach \cref{line:test:if:already:bundle}. 
			Because $p_i$ has included a non-$\bot$ second fragment in all its \bundle message, any of the (c-d) processes of $\bundleReceiveSet$ that receive one of $p_i$'s \bundle messages and has not already sent a \bundle message passes the condition at \cref{line:test:if:already:bundle}.
			%
			%    \FT{I've tried to unpack what was meant by `any such process', which was a bit elliptic IMHO.}%
			%they pass the condition at \cref{line:check:frag:not:bot}, and 
			%
			Each such process then disseminates a (valid) \bundle message at \cref{line:v3.1:bundle:with:bot}. This behavior
			yields $|\bundleSendSet|\geq c- {\Dadv}$. %By \cref{subobs:bundleR:implies:bundleS}, $|\bundleSendSet|\geq|\bundleReceiveSet|$, which yields the observation with the previous inequality.
		\end{obsProof}
		
		
		
		Let \bundleKReceiveSet be the set of correct nodes that receive \bundle messages from at least $\ECCthreshold$ distinct correct processes.

		\medskip
		\cref{subobs:counting:bundle:equation} is a detailed version of~\cref{subobs:Scounting:bundle:equation} in \cref{thm:SGlobal}.
  
		\begin{subobservation}\label{subobs:counting:bundle:equation}
			$|\bundleKReceiveSet|\times|\bundleSendSet| + (\ECCthreshold-1)(|\bundleReceiveSet|-|\bundleKReceiveSet|) \geq |\bundleSendSet|(c-\Dadv)$.
		\end{subobservation}
		
		%%%%%% FIGURE %%%%%%%%
		\begin{figure}[ht]
			\centering
			\input{fig/msg-dist}
			\caption{Distribution of distinct \bundle messages received by correct processes.
				The poof of Observation~\ref{subobs:bundleKReceiveSet:geq:frac} shows that $|\bundleSendSet|>\ECCthreshold-1$.}
			%\EMS{Please remind the reader why k-1<|Bsend| or say which Lemma shows this.}}
		\label{fig:msg_dist}
	\end{figure}
	%%%%%% FIGURE %%%%%%%%
	
	
	\renewcommand{\obscnt}{\ref{subobs:counting:bundle:equation}}
	\begin{obsProof}
		Let us denote by \numberBundleMsg the overall number of valid \bundle messages received by correct processes from distinct correct senders. More specifically, in the case when a correct node disseminates \bundle messages both at \cref{line:v3.1:bundle:comm,line:v3.1:bundle:with:bot}, we only consider the \emph{last} \bundle message, \ie the one of \cref{line:v3.1:bundle:comm}. 
		%
		We know that each $p\in \bundleSendSet$ sends a \bundle message, which by 
		%\cref{subobs:all:bundle:valid:hm} 
		\cref{lem:all:msgs:sent:valid}
		is valid. As the message adversary may drop up to~$\Dadv$ out of the $n$ messages of this $\comm$, we are guaranteed that at least $c-\Dadv$ correct nodes receive $p$'s \bundle message. This immediately implies that   
		\begin{equation}\label{eq:numberBundleMsg:geq}
			\numberBundleMsg \geq |\bundleSendSet|(c-\Dadv).
		\end{equation}
		
		% \ran{is the figure really needed?}\FT{It's a matter of preference I think: once you've understood the reasoning the figure is not needed, but it can helps to visualize things the first time}
		
		As illustrated in \cref{fig:msg_dist}, the processes in $\bundleKReceiveSet$ may receive up to $|\bundleSendSet|$ valid \bundle messages from distinct correct senders (one from each sender in $\bundleSendSet$), for a maximum of $|\bundleKReceiveSet|\times|\bundleSendSet|$ \bundle messages overall. The remaining process of $\bundleReceiveSet\setminus\bundleKReceiveSet$ may each receive up to $\ECCthreshold-1$ valid \bundle messages from distinct correct senders, by definition of $\bundleKReceiveSet$. 
		As $\bundleKReceiveSet\subseteq\bundleReceiveSet$ by definition, $|\bundleReceiveSet\setminus\bundleKReceiveSet|=|\bundleReceiveSet|-|\bundleKReceiveSet|$, and the processes of $\bundleReceiveSet\setminus\bundleKReceiveSet$
		accounts for up to $(\ECCthreshold-1)(|\bundleReceiveSet|-|\bundleKReceiveSet|)$ 
		%\EMS{is it $(|\bundleReceiveSet|-|\bundleKReceiveSet|)$ or $(|\bundleKReceiveSet|-|\bundleReceiveSet|)$? Please explain.}\FT{There was a typo in the previous sentence (now corrected), $\bundleKReceiveSet\setminus\bundleReceiveSet$ should have been $\bundleReceiveSet\setminus\bundleKReceiveSet$. I've also added a sentence to explain why $|\bundleReceiveSet\setminus\bundleKReceiveSet|=|\bundleReceiveSet|-|\bundleKReceiveSet|$.} 
		valid \bundle messages overall. As the \bundle messages counted by \numberBundleMsg are received either by correct processes in $\bundleKReceiveSet$ or in $\bundleKReceiveSet\setminus\bundleReceiveSet$, these observations lead to
		\begin{equation}\label{eq:numberBundleMsg:leq}
			|\bundleKReceiveSet|\times|\bundleSendSet| + (\ECCthreshold-1)(|\bundleReceiveSet|-|\bundleKReceiveSet|)   \geq \numberBundleMsg.
		\end{equation}
		
		Combining \cref{eq:numberBundleMsg:geq,eq:numberBundleMsg:leq} yields the desired inequality.
		%
	\end{obsProof}



		\medskip
		\cref{subobs:bundleKReceiveSet:geq:frac} is a detailed version of~\cref{subobs:SbundleKReceiveSet:geq:frac} in \cref{thm:SGlobal}.

 
	\begin{subobservation}\label{subobs:bundleKReceiveSet:geq:frac}
		%$\displaystyle|\bundleKReceiveSet| \geq c\left(1-\frac{\Dadv}{c-\ECCthreshold+1}\right).$
		$\displaystyle |\bundleKReceiveSet| \geq c - \Dadv\left(\frac{1}{1-\left(\frac{\ECCthreshold-1}{c-\Dadv}\right)}\right).$
	\end{subobservation}
	
	
	
	
	\renewcommand{\obscnt}{\ref{subobs:bundleKReceiveSet:geq:frac}}
	\begin{obsProof}
		%\cref{subobs:counting:bundle:equation} yields by a simple transformation
		Rearranging the terms of~\cref{subobs:counting:bundle:equation}, and recalling that $|\bundleReceiveSet|\leq c$ and $\ECCthreshold\ge 1$, we get
		\begin{equation}
			|\bundleKReceiveSet|\times(|\bundleSendSet|-\ECCthreshold+1) \geq |\bundleSendSet|(c-\Dadv) - |\bundleReceiveSet|(\ECCthreshold-1)  \geq |\bundleSendSet|(c-\Dadv) -c(\ECCthreshold-1).
		\end{equation}
		%  As $|\bundleReceiveSet|\leq c$ and $\ECCthreshold\geq 1$, the above equation yields
		% \begin{equation}
			%   |\bundleKReceiveSet|\times(|\bundleSendSet|-\ECCthreshold+1) \geq |\bundleSendSet|(c-\Dadv) -c(\ECCthreshold-1).
			%  \end{equation}
		By \cref{subobs:bundleR:and:bundleS:geq:c-d} and \cref{asm:MBRBassumptionR}, $|\bundleSendSet| \geq c-\Dadv \geq c-2 \Dadv\geq \ECCthreshold$, therefore $|\bundleSendSet|-\ECCthreshold+1>0$, and the previous equation can be transformed in
		\begin{equation}\label{eq:bundleKReceiveSet:geq}
			|\bundleKReceiveSet| \geq
			\frac{|\bundleSendSet|(c-\Dadv)-c(\ECCthreshold-1)}{|\bundleSendSet|-\ECCthreshold+1}.
		\end{equation}
		Note that the right-hand side of \cref{eq:bundleKReceiveSet:geq} is a monotone increasing function in~$|\bundleSendSet|$ when $|\bundleSendSet|>\ECCthreshold-1$, as its derivative, %w.r.t~$\bundleSendSet$, %
		$\frac{\Dadv(\ECCthreshold+1)}{(|\bundleSendSet|-\ECCthreshold+1)^2}$, is positive.
		By \cref{subobs:bundleR:and:bundleS:geq:c-d}, $|\bundleSendSet|\in [c-\Dadv, c]\subseteq[\ECCthreshold,c]$. 
		% OLD VALUE when function was assumed decreasing
		% The minimum of the righ-hand side of \cref{eq:bundleKReceiveSet:geq} is therefore obtained for $\bundleSendSet=c$, yielding
		%   \begin{equation}
			%   |\bundleKReceiveSet| \geq
			%   \frac{c(c-\Dadv-\ECCthreshold+1)}{c-\ECCthreshold+1} =
			%   c\left(1-\frac{\Dadv}{c-\ECCthreshold+1}\right).
			% \end{equation}
		The minimum of the right-hand side of \cref{eq:bundleKReceiveSet:geq} is therefore obtained for $\bundleSendSet=c-\Dadv$, yielding
		\begin{equation}
			|\bundleKReceiveSet| \geq
			\frac{(c-\Dadv)^2-c(\ECCthreshold-1)}{(c-\Dadv)-\ECCthreshold+1}
			= c - \Dadv\left(\frac{1}{1-\left(\frac{\ECCthreshold-1}{c-\Dadv}\right)}\right).
		\end{equation}
	\end{obsProof}


	\medskip
	\cref{subobs:all:bundleKReceiveSet:mbrb:deliv:m} is a detailed version of~\cref{subobs:Sall:bundleKReceiveSet:mbrb:deliv:m} in \cref{thm:SGlobal}.

 
 
	\begin{subobservation}\label{subobs:all:bundleKReceiveSet:mbrb:deliv:m}
		All nodes in $\bundleKReceiveSet$ MBRB-deliver~$m$.
	\end{subobservation}
	
	\renewcommand{\obscnt}{\ref{subobs:all:bundleKReceiveSet:mbrb:deliv:m}}
	\begin{obsProof}
		Consider $p_u\in \bundleKReceiveSet$. By the definition of $\bundleKReceiveSet$, the node~$p_u$ receives $\ECCthreshold$ valid \bundle messages from $\ECCthreshold$ distinct correct processes. Let us denote by $\langle \bundle,\allowbreak h_x, (\tilde m_x,\pi_x,x), \bull, \sigsset_x \rangle $ these $\ECCthreshold$ messages with $x\in[\ECCthreshold]$. By \cref{subobs:all:bundle:valid:hm}, for all $x\in[\ECCthreshold]$, $h_x=h_m$. In addition, each $\sigsset_x$ contains strictly more than $(n+t)/2$ valid signatures for $h_m$. As a result, $p_u$ eventually stores strictly more than $(n+t)/2$ valid signatures for $h_m$.
		
		Because the messages are valid, so are the proofs of inclusions $\pi_x$, and as we have assumed that the Merkle proofs of inclusion are fragment collision-resistant, $h_x=h_m$ implies that the received fragments $\tilde m_x$ all belong to the set of fragments computed by \psender at \cref{line:fragments:for:m} for $m$. As the \bundle messages were received from $\ECCthreshold$ distinct correct processes, the node~$p_u$ receives at least $\ECCthreshold$ distinct valid fragments for $m$ during its execution.
		%
		%\FT{This last claim only holds if correct processes check they are receiving the fragment they are meant to receive, which they do not explicitly do at the moment. All fragments are checked to be valid, but a Byzantine process could `mix' them up by sending valid fragments to the wrong processes. Can proofs of inclusion also encode the position/index of a fragment? Possibly if the concatenation operation used for internal Merkle tree nodes does not commute (??).}
		%\ran{AFAIU, the index/position is built-in in the Merkle tree and we get it for free. The reason is that $hash(a \| b) \ne hash(b \|a)$, so you must order the hashes correctly, or otherwise the concatenation of two hashes in a certain layer will yield the incorrect output; I changed the proof to explicitly include the index, which corresponds to the \EMS{What is party number?}\FT{That's the process id} party number, \ie $(m_i,\pi_i,i)$.}\FT{It looks like this closes this issue I think.}
		%
		If $p_u$ has not MBRB-deliver any message yet, the condition at \cref{line:quorum:sigs:enough:fragments} eventually becomes true for $h_m$, and $p_u$ reconstructs $m$ at \cref{line:v3.1:reconstruct:m}, since it possesses at least $k$ (correct) message fragments, which are sufficient for the correct recovery of~$m$ by our choice of ECC. %(\cref{sec:ECC-instantiation}). 
        Then, $p_u$ MBRB-delivers $m$ at \cref{ln:MBRBdeliverMjSn}.
		%
		On the other hand, if $p_u$ has already MBRB-delivered some message~$m'$,
		%when the condition at \cref{line:quorum:sigs:enough:fragments} becomes true for~$h_m$, 
		then \cref{thm:duplicity} (MBRB-No-duplicity) implies $m'=m$, since 
		$p_i$ is known to have MBRB-delivered~$m$. 
		Therefore, in all possible cases, $p_u$ MBRB-delivers~$m$.
	\end{obsProof}
	
	\cref{thm:Global} follows from \cref{subobs:bundleKReceiveSet:geq:frac,subobs:all:bundleKReceiveSet:mbrb:deliv:m} and the fact that all nodes in $\bundleKReceiveSet$ are correct.
\end{lemmaProof}	

% REMOVED FROM PODC's SUBMISSION

\remove{

\Subsection{Communication analysis}
\label{sec:complexity}
This section proves the communication part of our main \cref{thm:main}. Specifically, we prove the following. 
%
%\ran{is it too redundant to repeat it as a lemma?}\FT{It's fine by me.}
%
\begin{lemma}\label{lem:communication}
	%Given a correct sender, 
	The correct nodes in Algorithm~\ref{alg:3.1:merkle:trees} collectively
	communicate at most~$4n^2$ messages. Each correct node communicates at most $O(|m| + n^2\kappa)$ bits. Overall, $O(n|m| + n^3\kappa)$ bits are communicated. 
\end{lemma}
\renewcommand{\lemcnt}{\ref{lem:communication}}
\begin{lemmaProof}
	Let us begin by counting the messages communicated during an instance of \cref{alg:3.1:merkle:trees}. 
	To that end, we count $\comm$ and $\broadcast$ invocations throughout the algorithm execution.
	The sender,~\psender, initiates the execution by sending \send messages at \cref{ln:v3.1:commV1ldotsVn}.
	In Phase~I, each correct node that has received a \send message broadcasts a \forward message once (\cref{line:v3.1:bcast:forward,line:condition:sign:hash:SEND}). 
	However, if it first receives a \forward before the \send arrives, it performs one additional broadcast of \forward messages (\cref{line:v3.1:forward:after:forward}). 
	This yields at most $2$ $\comm$ and $\broadcast$ invocations per correct node until the end of Phase~I. We can safely assume that a correct sender always sends a single \forward (i.e., it immediately and internally receives the \send message sent to self); thus $\psender$ is also limited to at most $2$ invocations up to this point.
	
	In Phase~II, each correct node that MBRB-delivers a message at \cref{ln:MBRBdeliverMjSn} transmits \bundle messages at \cref{line:v3.1:bundle:comm}.
	This can only happen once due to the condition at \cref{ln:bulljsnWasNotMBRBdelivered}.
	%\FT{Terminology: We use `broadcast' both for lines using $\comm$ and for those using $\broadcast$, which can be confusing. We could use a generic term such as `disseminate' that is not linked to any of the 2.}%
	Additionally, it may transmit \bundle messages also at \cref{line:v3.1:bundle:with:bot}, upon the reception of a \bundle. 
	However, this second \bundle transmission can happen at most once, due to the if-statement in \cref{line:test:if:already:bundle}.
	This leads to at most $2$ additional $\comm$ and $\broadcast$ invocations, per correct node.
	
	Thus, as the number of correct nodes is bounded by~$n$, the two phases incur in total at most $4n$ invocations of $\comm$ and $\broadcast$ overall. 
	Since each such invocation communicates exactly $n$ messages, the total message cost
	for correct processes when executing one instance of \cref{alg:3.1:merkle:trees}
	%, during a single execution of \cref{ln:v3.1:commV1ldotsVn}, 
	is upper bounded by~$4n^2$.
	%\FT{I've replaced `during a single execution of \cref{ln:v3.1:commV1ldotsVn}' with the formulation above, as the analysis holds even if \psender is dishonest.}%
	Note that the above analysis holds for correct nodes also in the presence of Byzantine participants, including when \psender is dishonest.
	%\FT{Please CHECK you agree.}%
	%\ran{Thanks, I thought about it when writing it. Actually, the sender only sends FORWARD once because it will always get its own SEND before he gets FORWARD. I thought this is too fine detail to bother to mention, but the summary that every node (including sender) sends 2n messages up to the end of phase I is correct}\FT{`it will always get its own SEND before he gets FORWARD': I think this assumes a node always gets its own broadcast despite the MA. It makes complete sense in practice, but formally we don't say so explicitly in \cref{sec:messageAdversary} when defining the MA. Should we add a note either here or there on this point?}
	
	We now bound the number of bits communicated by correct nodes throughout a single instance of \cref{alg:3.1:merkle:trees}.
	Consider Algorithm~\ref{algo:computeFragmentMerkleTree}. 
	Let $m$ be a specific application message. 
	We have $|\tilde m|=O(|m|)$ since we use a code with a constant rate. %; see \cref{sec:ECC-instantiation}. 
	Thus, any specific fragment $\tilde m_i$ has length $|\tilde m_i| = O(|m|/n)$.
	Recall that both the size of a signature and of the hash is $O(\kappa)$~bits (\cref{sec:crypto-prim}).
	It is important to note that along the signatures, we also include the identifier of the singing node, which takes additional $O(\log n)$~bits. 
	However, since we assume $\kappa=\Omega(\log n)$, 
	%\EMS{Rev. \#3 says 'Up until this point, you have assumed $\kappa = \Omega(\log n)$; perhaps keep that notation instead of the $\kappa > \log n$ invocation here for consistency, since these are not identical?'}%
	%\FT{I agree.}%%\EMS{Ran, may I kindly ask you to help with updating the proof?}
	%
	the inclusion of this field does not affect asymptotic communication costs.
	The Merkle tree construction (\cref{sec:merkle}) implies that for any $j\in [n]$, the Merkle proof~$\pi_j$ has length $|\pi_j|=O(\kappa \log n)$.
	
	We now turn to trace all the $\comm$ and $\broadcast$ instances in \cref{alg:3.1:merkle:trees} and analyze the number of bits communicated in each.
	The \send $\comm$ in \cref{ln:v3.1:commV1ldotsVn} communicates $n$ messages, where each message includes a fragment of the application message ($O(|m|/n)$ bits) along with its Merkle proof ($O(\kappa \log n)$ bits), a hash ($O(\kappa)$ bits), and a signature  ($O(\kappa)$ bits). Thus, the sender communicates at most $O(|m|+ \kappa n \log n)$ bits by this operation. 
	Each \forward broadcast in lines~\ref{line:v3.1:bcast:forward} and~\ref{line:v3.1:forward:after:forward} sends $n$ copies of a message, where each message includes: a hash ($O(\kappa)$ bits), at most one application message fragment in addition to its Merkle proof ($O(|m|/n+ \kappa\log n)$ bits), and two signatures ($O(\kappa)$ bits).
	Hence, each one of lines~\ref{line:v3.1:bcast:forward} and~\ref{line:v3.1:forward:after:forward} communicates a total of $O(|m| + \kappa n\log n)$ bits.
	The \bundle communication in lines~\ref{line:v3.1:bundle:comm} or~\ref{line:v3.1:bundle:with:bot} sends $n$ messages, where each contains a hash ($O(\kappa)$ bits), at most two application message fragments in addition to their Merkle proof ($O(|m|/n+ \kappa\log n)$ bits), and up to $n$ signatures ($O(\kappa n)$ bits). Hence, each of these lines communicates at most $O(|m|+n^2\kappa)$ bits.
	As analyzed above, the sending process (\psender, when correct) 
	performs at most one $\comm$ of \send messages, while each correct node performs at most two $\broadcast$ of \forward messages, and at most two $\comm$/$\broadcast$ of \bundle messages. 
	% each node performs at most one $\comm$ of \send messages, at most two $\broadcast$ of \forward messages, and at most two $\comm$ of \bundle messages. 
	Thus, each node communicates at most $O(|m| + n^2\kappa)$ bits.
	%\FT{Please CHECK: I've changed the above sentence to stress that among correct processes only \psender executes \cref{ln:v3.1:commV1ldotsVn}. (I don't think this changes the reasoning or the final result though; it is just more precise.)}
	Overall, the total bit communication by correct nodes during the execution of \cref{alg:3.1:merkle:trees} is $O(n|m| + n^3\kappa)$.
	As above, the analysis holds in Byzantine nodes' presence, even if \psender is dishonest.
	%\FT{Please CHECK you agree.}
\end{lemmaProof}

} % REMOVED FROM PODC's SUBMISSION

==> prelim.tex <==
\Section{Preliminaries}
\label{sec:prelim}
\B
\Paragraph{General notations and conventions}
For a positive integer~$n$, let $[n]$ denote the set $\{1,2,\ldots,n\}$. A sequence of elements $(x_1,\ldots,x_n)$ is shorthanded as $(x_i)_{i\in[n]}$. We use the symbol~`$\bull$' to indicate any possible value. 
That is, $(h,\bull)$ means a tuple where the second index includes any arbitrary value which we do not care about. %\EMS{MR said 'page 4, section 2 line 3:   a vector  -->  a pair ?'}
All logarithms are base 2.
	
\Subsection{Nodes and Network} 
We focus on asynchronous message-passing systems that have no guarantees of communication delay. 
Also, the algorithm cannot explicitly access the clock or use timeouts. 
The system consists of a set, $\sP=\{ p_1, \ldots, p_n\}$, of $n$ fail-prone nodes (or processes).
We identify party~$i$ with~$p_i$. 
		
\Paragraph{Communication means} 
Any ordered pair of nodes $p_i,p_j \in \sP$ has access to a communication channel, $\mathit{channel}_{i,j}$.
%
Each node can send messages to all nodes (possibly \ta{by} sending a different message to each node).
That is, any node, $p_i\in \sP$, can invoke the transmission macro, $\comm(m_1,\ldots, m_n)$, that communicates the message $m_j$ to~$p_j$ over $\mathit{channel}_{i,j}$.
The message~$m_j$ can also be empty, in which case nothing will be sent to~$p_j$.
However, in our algorithms, all messages sent in a single $\comm$ activation will have the same length.
%%OLD: Each message~$m_j$ must be non-empty, and we assume these messages have the same length.
%
Furthermore, when a node sends the same message $m$ to all nodes, we write $\broadcast(m)=\comm(m,m,\ldots,m)$ for shorthand.
We call each message $m_j$ transmitted by the protocol an \emph{implementation message} (or simply, a \emph{message}) to distinguish such messages from the \emph{application}-level messages, \ie the one the sender wishes to broadcast\reduce{ reliably}. 


\Paragraph{Byzantine nodes} 
%
\label{sec:nodeFailures}
Faulty nodes are called \emph{Byzantine}, and their adversarial behavior can deviate from the proposed algorithm in any manner.
For example, they may crash (by stopping sending messages) or send fake messages,  deviating from the protocol.
Their ability to communicate, and collude is unlimited.
They might perform any arbitrary computation, and we assume their computing power is at least as strong as that of non-faulty nodes, yet not as strong as to undermine the security of the cryptographic signatures we use \ta{(see \Cref{sec:crypto-prim})}.
We assume that at most $t$ nodes are faulty, where $t$ is a value known to the nodes.  
Non-faulty nodes are called \emph{correct nodes}. 
The set of correct nodes
contains $c$ nodes where $n-t \leq c \leq n$. 
The value of $c$ is unknown.

% to correct nodes

%\EMS{Try to see if you can replace '(see below)' with a section number. Also, I understand the need to limit the computational power of Byzantine nodes. But, what about their ability to coordinate? For example, is there one adversary that controls the scheduling, the message delivery, and the actions of the Byzantine nodes? Or is it a distributed system by itself subject to all the impossibilities in the area of distributed computing? How about not making any limit on their ability to coordinate and their computational power except an explicit assumption that they (or the adversary) cannot 'undermine the security of the cryptographic signatures'.}
 
Faulty nodes may deviate arbitrarily from the correct implementation of $\commP$. For instance, they may unicast messages to only a subset of the nodes in~$\sP$.
%
As mentioned, each pair of nodes can communicate  using~$\mathit{channel}_{i,j}$.
While $\mathit{channel}_{i,j}$ is assumed to be a reliable channel that is not prone to message corruption, duplication, reordering, or the creation of fake messages that were never sent by nodes;
the \emph{message adversary}~\cite{SW89,DBLP:journals/tcs/SantoroW07,DBLP:reference/algo/Raynal16a}, which we specify next, has a limited ability to cause message loss.

\Paragraph{Message adversary} 
%
\label{sec:messageAdversary}
%
This entity can remove implementation messages from the communication channels used by correct nodes when they invoke~$\commP$. 
More precisely, during each activation of $\comm(m_1,\ldots,m_n)$, the adversary has the discretion to choose up to ${\Dadv}$ messages from the set~$\{m_i\}$ %_{i \in [n]}$
and eliminate them from the corresponding communication channels where they were queued. We assume that the adversary has full knowledge of the contents of all messages~$\{m_i\}$, and thus it makes a worst-case decision as to which messages to eliminate.

The failures injected by a message adversary differ from those of classical sender and/or receiver omission\reduce{ failure}s in that they are \emph{mobile}.
\Ie they are not pinned to a set of particular nodes but may move between any correct nodes during the same execution since they are defined per invocation of~$\commP$. 
In particular, no\reduce{ correct} node is immune to the message adversary.

Note that for the case of ${\Dadv} = 0$, the adversary is as weak as the common settings in which all communication channels are reliable (since no message is ever lost) and $t$ nodes are Byzantine.
Assumption~\ref{asm:MBRBassumption} limits the adversary's power in order to avoid network partitions.
As mentioned above, this is a necessary requirement on any MBRB algorithm~\cite{AFRT23}. 

%\EMS{Maybe we should add the following sentence to the TR version 'But, for ${\Dadv}>1$, the message adversary is stronger since it needs to cover cases related to silent churn, for example, when nodes decide to disconnect from the network (without the provision of notification).'}
\B
\begin{assumption}[Adversary-power-assumption]
\label{asm:MBRBassumption}
$n > 3t$+$2{\Dadv}$.
\end{assumption}	
\B
Since the message adversary can omit all implementation messages that are sent to a given set $D\subseteq \sP:|D|={\Dadv}$, we know that $\ell$, the number of correct nodes that are guaranteed to output the broadcast~$m$ correctly, must satisfy $\ell \leq c-{\Dadv}$. 
Nevertheless, the message adversary cannot partition the network since $n > 2{\Dadv}$. 



Such a hybrid fault model has been investigated in the past in synchronous networks~\cite{DBLP:journals/tcs/BielySW11}, but has remained little studied in an asynchronous setting, except for the work of Schmid and Fetzer~\cite{DBLP:conf/srds/SchmidF03} that limits itself to round-based algorithms (unlike us) and does not cover full disconnections \ft{of correct nodes} (which we do).
Modeling the full disconnection of correct nodes is relevant in practice, as this captures correct processes that remain disconnected for long periods.
%
In addition to bounding the maximal number of outgoing messages that a correct sender might lose (as we do), the model proposed by Schmid and Fetzer~\cite{DBLP:conf/srds/SchmidF03} also bounds the maximal number of incoming messages that any correct process might miss.
Although this adds an elegant symmetry into the model, such a choice poses significant challenges when considering asynchronous networks since there is no obvious scope, such as a synchronous round, on which to limit the number of incoming messages missed by a given process. The solution adopted by Schmid and Fetzer~\cite{DBLP:conf/srds/SchmidF03} consists in restricting the fault model to round-based algorithms. We chose to avoid such constraints to allow algorithms that do not follow this structure.


% Original text by Elad
%\ems{One can envision a message adversary model with a bound on the minimal number of incoming messages that any given process might receive to model the full disconnection of correct nodes. In the context of real-world systems, such a model would represent correct processes that remain disconnected for long periods. These approaches pose significant challenges when considering asynchronous networks since there is no obvious scope, such as a synchronous round, on which to limit the number of incoming messages missed by a given process. One option would be to restrict our model to round-based algorithms, as done by Schmid and Fetzer~\cite{DBLP:conf/srds/SchmidF03}. However, we chose to avoid such constraints to allow algorithms that do not follow this structure.}

\newcommand{\nECC}{{\bar n}}
\newcommand{\kECC}{{\bar k}}
\newcommand{\rECC}{{\bar r}}
\newcommand{\dECC}{{\bar d}}

\Subsection{Error Correction Codes} 
\label{sec:ecc}
%
A central tool used in our algorithm is an error-correction code (ECC)~\cite{roth06}. Intuitively speaking, an ECC takes a message as input and adds redundancy to create a codeword from which the original message can be recovered
even when parts of the codeword are corrupted. 
%
In this work, we focus on \emph{erasures}, a corruption that replaces a symbol of the codeword with a special erasure mark~$\bot$.  


Let $\F$ denote a finite field whose size we set later, and let $\bot$ be a special symbol~$\bot \notin \F$. 
% \TA{Shouldn't we write $\F^q$ here instead so that readers not familiar with finite fields understand that the superscript in later notations refers to the size of the field?}\ran{GF(q) is a standard notation; $F^q$ means something else}
Given two strings of the same length, $x,y \in \F^n$, their \emph{Hamming distance} is the number of indices where they differ, $\Delta(x,y) = | \{i\in[n] \mid x_i \ne y_i\}|$. Given a subset $I \subseteq [n]$, we denote by $x_I \in \F^{|I|}$ the string $x$ restricted to the indices in~$I$.

To avoid confusion with global parameters, we denote the ECC-specific parameters by using a bar (\eg $\bar x$).
An \emph{error-correction code} is a function $\ECC : \F^\kECC \to \F^\nECC$, with \emph{rate}  $\rECC=\kECC/\nECC$, and \emph{distance} ${\dECC} =  \min_{x,y\in \F^\kECC, x\ne y} \dist( \ECC(x), \ECC(y))$.
%
%\emph{Linear} codes are such that their image is a linear subspace of~$\F^n$ of dimension~$k$. 
The Singleton bound determines that $\dECC\le \nECC-\kECC+1$, and when the equality holds, 
the code is said to be maximum distance separable (MDS).
A prominent example of MDS codes is Reed-Solomon (RS) codes~\cite{RS60}, which exist for any $\kECC,\nECC$, and $|\F|\ge \nECC$. Such codes can be efficiently encoded and decoded~\cite{roth06}.
%
The erasure correction capabilities of a code depend on its distance, as given by the following fact.

% cf. Fact~\ref{fct:CC} for correcting substitutions and Fact~\ref{fct:ErasureECC} for correcting erasures.
% \begin{fact}[Substitution Correction Capability]
%     %
%     \label{fct:CC}
%     %
%     Any error correction code of distance ${d}$ can recover up to $\lfloor (d-1)/2 \rfloor$ substitutions. 
%     That is, for any $y\in \F^n$ there exists at most a single $x\in \F^k$ such that 
%     $\dist(\ECC(x),y) < {d}/2$.  
% \end{fact}

\B
\begin{fact}[Erasure Correction Capability]
    \label{fct:ErasureECC}
    Any error-correction code of distance ${\dECC}$ can recover up to ${\dECC}-1$ erasures. 
    That is, for any $y\in (\F\cup \{\bot\})^\nECC$, let $E = \{ i \mid y_i = \bot\}$ the set of erased indices. Then, if $|E|<{\dECC}$, there is at most a single $x\in \F^\kECC$ such that 
    $y_{[\nECC]\setminus E}=\ECC(x)_{[\nECC]\setminus E}$.  
\end{fact}
\B

\Subsection{Cryptographic Primitives} \label{sec:crypto-prim}
Our algorithm relies on cryptographic assumptions. 
%
%Towards that end, w
%
We assume that the Byzantine nodes are computationally bounded with respect to the security parameter, denoted by~$\kappa$. That is, all cryptographic algorithms are polynomially bounded in the input~$1^\kappa$.
%\FT{What is the semantic of $1^\kappa$? Is it the same as $\{0,1\}^\kappa$}\ran{It is common in complexity to measure time as a function of the length of the input; so here the input is a string of length $\kappa$, which is the base unit for complexity computation. It is the all-ones string, by convention.} 
We assume that $\kappa =\Omega$($\log n$).
%
We further assume the availability of Public Key Infrastructure (PKI), which is the setting that assumes each party is assigned a pair of public/private keys, generated according to some common key-generation algorithm. Further, at the start of the computation, each party holds its own private key and the public key of all other parties. This setting implies private and authenticated channels.
In particular, 
each party has public and private keys to support the following cryptographic primitives.


\Subparagraph{Hash functions}
\label{sec:hash}
A collision-resistant hash\reduce{ function} is a function\footnote{Formally speaking, a hash function must be chosen randomly from a family of possible hash functions. Otherwise, an adversarial algorithm~$A$ exists. We avoid a formal treatment of this issue in our paper. In practice, a fixed function is used (\eg SHA2 or SHA3).}
$\Hash: \{0,1\}^* \to \{0,1\}^\kappa$ that satisfies the following
%\begin{enumerate}
%\item 
\emph{collision resistance} property:
For any computationally bounded algorithm $A$ and any $x\in \{0,1\}^*$,
\( \Pr [A(x) = x' \wedge \Hash(x')=\Hash(x)]<2^{-\Omega\text{(}\kappa\text{)}}
\).
%Namely, 
%
\Ie finding a pair $x,x'$ with the same hash is infeasible, except with negligible probability in the security parameter.
%\end{enumerate}


\Subparagraph{Signature schemes}
%
\label{sec:cryptographicSignatures}\label{sec:signatures} 	
%
A \emph{digital signature} scheme is a pair of possibly randomized algorithms $\SIG = (\SIGN,\VER)$.
\TA{Why is $\VER$ capitalized and not $\SIGN$?}
The signing algorithm executed by node~$p_i$ (denoted, $\SIGN_i$) takes a message~$m$ and implicitly a private key.
It then produces a signature $\sigma = \SIGN_i(m)$.
The verifying algorithm takes a message, its corresponding signature, and the identity of the signer (and implicitly a public key), and outputs a single bit,  $b=\VER(m,\sigma,i)$, which indicates whether the signature is valid or not, $b \in \{\valid,\invalid\}$.
The signature scheme is parameterized by a security parameter~$\kappa$ and the following holds:
\begin{enumerate}%[topsep=0.25ex,itemsep=1.0ex]
\item \textbf{Validity:}
For any $m$ and $i\in [n]$, 
$ \VER (m, \SIGN_i(m),i) = \valid$.
\item \textbf{Unforgeabilty:}
for any $i\in[n]$ and for any computationally bounded algorithm $A$ that can access $\SIGN_i(\cdot)$ multiple times, let $\sigma = A(m)$ be the output of $A$ on some input~$m$, restricted to the case that $A$ cannot query $\SIGN_i(\cdot)$ on~$m$. 
It holds that
$\Pr [\VER(m,\sigma,i)=\valid]< 2^{-\kappa}$. 
The probability is over the randomness of the key (where the public key of~$p_i$ is given to~$A$, but the secret key is not) and the randomness of $\SIGN$ and~$A$.
\end{enumerate}
%
The signature size, $|\sigma|=\bigO{\kappa}$, is independent of the size of the signed message, $m$.
Common signature scheme\reduce{ implementations} are the BLS~\cite{BLS04}, the ECDSA~\cite{JMV01}, and the Schnorr~\cite{schnorr91} schemes.
%Also note that the adversary~$A$, and hence the Byzantine nodes, are assumed to be computationally bounded (in the security parameter~$\kappa$). 

% \begin{remark}\label{rem:signatureLength}
% In the rest of this work, we will assume that $\kappa > c_\kappa \log n$, for~$c_\kappa$ a constant. In this case, there is at most a polynomially-small probability for the adversary to forge a signature.
% \FT{Possible notation clash with $c$, the number of effectively correct nodes. Possibly replace by $K$ or $C$?}\ran{fixed}
% Union bounding over the polynomially many signatures generated and communicated throughout the execution of our schemes, we can assume that any signature that passes the verification is indeed authentic. 
% All of our theorems in this work are implicitly conditioned on this event, and thus hold with high probability. 
% \end{remark}


%\EMS{I cannot finish reading the text about 'Merkle Trees' since the parameter $t$ is used as the number of leaves but earlier $t$ was defined as the number of Byzantine nodes in the system.}
%\ran{I set a macro for this notation,change it as you wish. We only use $n$ fragments, so maybe we can use $n$ instead.}


\newcommand{\merkleFragments}{n} % {{\tilde t}}

\Subparagraph{Merkle Trees~\cite{Merkle90} }
\label{sec:merkle}
These are means to commit to a message composed of several fragments so that one can prove, for each fragment independently, that it\reduce{ indeed} belongs to the committed message. 
Formally, this primitive is parameterized by a security parameter~$\kappa$ and consists of two functions: $\MerkleTree(\cdot)$ and $\MerkleVerify(\cdot)$ that work as follows.
For any vector of strings, $x_1,\ldots,x_\merkleFragments = (x_i)_{i\in[\merkleFragments]}$ the function 
$(h, \pi_1, \ldots, \pi_\merkleFragments) \gets \MerkleTree(x_1,\ldots, x_\merkleFragments)$ 
returns $h$---the hash of the Merkle tree, and $\pi_i$---a proof of inclusion for $x_i$.
The following hold.
\begin{enumerate}%[topsep=0.25ex,itemsep=1.0ex]
    \item \textbf{Proof of inclusion:}
    Let $(h, (\pi_i)_{i\in[\merkleFragments]}) = \MerkleTree(x_1,\ldots, x_\merkleFragments)$. Then for any $i\in[\merkleFragments]$, it holds that $\MerkleVerify(h,\pi_i,x_i,i)=\valid$.
    %
    \item \textbf{Fragment collision-resistance:}
    \sloppy
    For any $j\in[\merkleFragments]$ and any randomized algorithm $A$ that is given  $(x_i)_{i\in[\merkleFragments]}$ and $(h, (\pi_i)_{i\in[\merkleFragments]}) = \MerkleTree(x_1,\ldots, x_\merkleFragments)$ as an input, 
    $\Pr[A \text{ outputs } (x_j',\pi'_j,j) \wedge  \MerkleVerify(h,\pi'_j,x_j',j)=\valid] < 2^{-\Omega\text{(}\kappa\text{)}}$.
    Namely, it is difficult to generate $x_j'\ne x_j$ along with a proof~$\pi_j'$ that passes the proof of inclusion concerning the same~$h$. 
%     \EMS{Rev. \#2 says: '$Pr[A~outputs~ (x_j', \pi_j, k)]$ ---> should be  $\pi'_j$ instead of  $\pi_j$}%
%     \FT{I think Rev. \#2 is correct. Algorithm $A$ outputs a new proof $\pi'_j$ along with the `fake' element $x_j'$, i.e. it outputs $(x_j',\pi'_j,j)$ and not $(x_j',\pi_j,j)$. }
% %
% \EMS{Ran, can you suggest what to do here?}\ran{corrected as the reviewer correctly suggests}
\end{enumerate}

%The construction of $\MerkleTree$ creates a
\Fs
A $\MerkleTree$ has a binary tree of hashes where the $\merkleFragments$ leaves are labeled with~$\Hash(x_i)$, and any internal node is labeled with the hash value of the labels of its children. The value~$h$ is the hash value at the root. The proof of inclusion~$\pi_i$ includes the labels of all nodes, which are siblings of nodes along the path from the root to the leaf~$\Hash(x_i)$; see~\cite{Merkle90}.
%We note that t
The value~$h$ is a collision-resistant hash of $(x_i)_{i\in[\merkleFragments]}$. Namely, given $(x_i)_i$ it is difficult to find $(y_i)_i \ne (x_i)_i$ such that $h_y=h_x$, where $h_x$ and $h_y$ are the roots of the Merkle trees for $(x_i)_i$ and $(y_i)_i$, respectively.
The tree construction allows reducing the total length of the hashes saved to prove the inclusion of some $x_i$. I.e., instead of saving one hash per fragment~$x_i$, totaling with $\merkleFragments\cdot \kappa$ bits, 
the above scheme features $|h|=\kappa$, and $|\pi_i|=\bigO{\kappa \log \merkleFragments}$ for any $i\in[\merkleFragments]$.

==> sec-intro_compacted.tex <==

\section{Introduction}
%	
\emph{Reliable Broadcast} allows $n$ asynchronous nodes to agree on a message sent by a designated node, the \emph{sender}, despite the possible malicious behavior of some of the nodes and the transmission network. 
Reliable broadcast plays a crucial role in several key applications, including consensus algorithms, replication, event notification, and distributed file systems, among others.
\ta{These systems sometimes require broadcasting large messages or files (\eg permissioned blockchains), and thus, reducing the communication overhead to a minimum is an important aspect of achieving scalability.}
% \FT{We could also mention , in 
% which blocks can be quite large (although, admittedly, some approaches have been proposed to decouple agreement on a block from its diffusion, e.g. in HoneyBadger.).}
% \TA{Yes but as we have seen before, sending the whole message and r-broadcasting the hash of this message at the same time 2 is not optimal for our case, because it gives a delivery power of $c-2d$. Maybe HoneyBadger would have the same problem of weak termination guarantees if there was an MA.}
In that vein, this work aims at providing \emph{communication efficient} solutions for the task of reliable broadcast in the presence of node and link faults.
%\TA{I would replace "consistency guarantees" with "fault-tolerance guarantees". The consistency guarantees stay the same (it is still a reliable broadcast), but the fault-tolerance guarantees get stronger (MA+Byz), no?}
%\ran{IMHO, it is too early to reach this point here. What fits here is a (vague) statement that our focus is BRB and reducing its communication. the rest should appear later. I changed accordingly}

%
%(e.g., in the case of broadcast-based distributed file systems), 


\emph{Byzantine} nodes~\cite{lamport1982byzantine,Dolev82} are faulty processes that are assumed to act cooperatively in an arbitrary manner to hinder the non-faulty nodes (also known as correct nodes) from reaching an agreement on the value of a sent message.
These faulty nodes can manifest in various ways, such as delivering fake messages that were never sent, altering the payload of messages sent by any faulty nodes, delaying message delivery, or even omitting messages altogether. Also, \ta{a} Byzantine failure can present itself differently to different nodes.

Solving reliable broadcast in the presence of Byzantine nodes (a problem known as BRB for Byzantine Reliable Broadcast), has been extensively studied for at least four decades. Bracha~\cite{DBLP:conf/podc/BrachaT83,DBLP:journals/jacm/BrachaT85} in particular showed that BRB could be implemented in asynchronous networks as soon as the number $t$ of Byzantine nodes is limited \ems{to be less than} a third of the nodes. This seminal result has since been followed by hundreds of works, with a various range of optimizations and tradeoffs between different parameters such as resilience, efficiency, and communication; see~\cite{DBLP:books/sp/Raynal18} for an excellent book on this topic.

A significant challenge to reliable broadcast algorithms arises when the message-passing system is unreliable and possibly cooperates with the $t$ Byzantine nodes. Link faults~\cite{SW89,DBLP:journals/tcs/SantoroW07} give Byzantine nodes (potentially limited) control over certain network links, enabling them to omit or corrupt messages \ft{(an ability captured under the umbrella term \emph{message adversary}~\cite{DBLP:reference/algo/Raynal16a})}.
This work focuses on \ft{a specific type of message adversary that} can only omit messages sent by correct nodes, but they cannot alter their content. 
\FT{After checking with Michel, I've rephrased the above to remove the idea that an MA is necessarily limited to message omissions.}%
The message adversary abstracts cases related to \emph{silent churn}, where nodes \ft{may} voluntarily or involuntarily disconnect from the network without explicitly notifying other nodes. 
During disconnection, the adversary causes correct nodes to pause the execution of their algorithm temporarily and resume upon reconnecting. 
In the message adversary model, correct nodes may miss messages sent over reliable communication channels by other nodes while they are disconnected, as there is no explicit notification about the message omission.

In a recent work~\cite{DBLP:journals/corr/abs-2205-09992}, Albouy, Frey, Raynal, and Taïani propose a reliable broadcast algorithm (which we denote \AFRT for short) for asynchronous networks, that withstands the presence of $t$ Byzantine nodes and a message adversary capable of omitting up to~$d$ messages per node's broadcast. 
To be more precise, a node communicates through a $\comm$ primitive (or a similar multicast/unicast primitive that targets a dynamically defined subset of processes),
%	
%\FT{In earlier submissions, some reviewers questioned the use of $\comm$ as possibly too restrictive. We could add a footnote to fend off the criticism, e.g.\footnote{\ft{Note that such a message adversary is not restricted to algorithms using the $\comm$ primitive. It can be equivalently defined for a multicast primitive that targets a dynamically defined subset of processes (be it multiple recipients or only one in the case of unicast), thus covering any message-passing algorithm.}}}; \EMS{I would prefer not to have footnotes, so I suggested a compromise.}\ran{not a strong feeling here, but I rather have footnotes when the message is somewhat divergent from the main idea. I am also fine with Elad's suggestion}
%\TA{I also like Elad's suggestion}%
%\FT{Yes, looks good to me as well.}
%	
which results in the transmission of~$n$ messages, with each node being sent one message, including the sender.
The message adversary can choose to omit messages in transit to a subset of at most $d$ \ft{correct} processes.
\FT{I've inserted \emph{correct}, as formally Byzantine processes are ignored in the definition of $d$.}%
The adversary is only limited by the size of that subset.
For instance, between different $\comm$ invocations, the adversary has the freedom to modify the set \ft{of correct processes} to which messages are omitted.
\AFRT guarantees the reliable delivery of any message when $n>3t+2d$. 
Moreover, they demonstrate the necessity of this bound on the number of Byzantine nodes and omitted messages, as no reliable broadcast algorithm exists otherwise.

One caveat of \AFRT regards its communication efficiency. 
While it achieves an optimal number of $O(n^2)$ messages, each node's communication requires $O(n\cdot(|m|+\log n+\kappa))$ bits, where $|m|$ represents the number of bits in the broadcast message, and $\kappa$ is the length of the digital signatures used in their algorithm. 
In this work, we revisit the task of MBRB and design an algorithm that significantly reduces the per-node communication \df{cost}, while preserving the total number of communicated messages.  \EMS{MR commented 'the total number of communicated messages ?? --> the total number of delivered ed messages'}\FT{Total number of messages sent by correct nodes? Byzantine nodes can send as many messages as they want. Or maybe this is obvious and does not need to be repeated each time.}\DF{Are we talking about the message complexity here or the number of delivered messages? I understood the former, and I believe message complexity would be clearer, as Michel clearly understood the latter.}
%
Our solution features at most~$4n^2$ messages \ta{sent by correct nodes}, and only $O(|m| + n^2\kappa)$ bits per \ta{correct }node.
Overall, $O(n|m| + n^3\kappa)$ bits are communicated \ta{by correct nodes}. 
Note that $\Omega(n|m| + n^2\kappa )$ serves as a straightforward lower bound on the overall communication (up to the size of the signature), see \eg \cite{nayak_et_al:LIPIcs:2020:13106}, as every \ta{correct} node must receive the message~$m$, and reliable broadcast of a single bit necessitates at least $\Omega(n^2)$ messages~\cite{DR85}.

\Subsection{Problem description}
%
\label{sec:probDesc}
%
We briefly describe the setting and problem of reliable broadcast and refer the reader to \cref{sec:prelim} for further details.
We assume $n$ nodes over an asynchronous network, where a message can be delayed for an arbitrary yet finite amount of time (unless omitted by the message adversary). 
We assume the existence of $t$ Byzantine nodes and a message adversary that can omit up to $d$ messages per invocation of the $\comm$ primitive. 
Furthermore, a designated sender node holds a message $m$ that it wishes to broadcast to all the nodes. 

An algorithm that satisfies the requirements of reliable broadcast despite Byzantine nodes and a message adversary is called a Message-adversary Byzantine Reliable Broadcast (\MBRB) algorithm.
The detailed version of \MBRB's requirements was formulated in~\cite{DBLP:journals/corr/abs-2205-09992}, see \cref{sec:MBRBdef}.
\df{We summarize them here as follows.}	\DF{Replaced this text: "We describe here some of the requirements that a reliable broadcast algorithm needs to satisfy."}
\textbf{(1)} For any sender invoking the broadcast algorithm, no two correct nodes deliver $m$ and $m'$, such that $m'\ne m$.
\textbf{(2)} If a correct sender broadcasts a message~$m$, at least $\ell$ correct nodes will deliver~$m$.
The quantity $\ell$ might depend on the adversary's power, \ie on $t$ and $d$.
\textbf{(3)} If a correct node delivers some message~$m$ from a correct sender, this correct sender has broadcast $m$ previously.

%\vspace*{-1em}
\Subsection{Contributions and techniques}
	
We present an \MBRB algorithm with near-optimal communication and delivery power~$\ell$.
\begin{theorem}[Main, informal]
\label{thm:main-informal}
For any~$\eps>0$, there exists an efficient \MBRB algorithm, such that every message~$m$ broadcast via this scheme is delivered by at least $\ell = n-t-(1+\eps)d$ correct nodes. 
%Further, if the broadcast is initiated by a faulty node, either no correct node delivers a message or at least $\ell$ correct nodes deliver \emph{the same} message. \ran{edited the last part, verify}  %%%% I am removing the last part. The Thm says this is an MBRB scheme, thus this property holds for sure. The above line only states its \ell and the below line the communication.
%
Each correct node sends  no more than $4n$ messages and communicates 
$O(|m|+n^2\kappa)$ bits overall, where $|m|$ is the length of the application message~$m$. 
\end{theorem}


We note that the above asymptotic communication holds assuming a sufficiently long message~$m$. 
Further, we note that $n-t-\Dadv$ is a natural upper bound on the deliver power~$\ell$ of any MBRB algorithm. This bound arises from the power of the message adversary to isolate a subset of the correct parties of size~$\Dadv$, and omit all messages sent to this subset. 
Our solution obtains a delivery power~$\ell$  that is as close to the limit as desired, at the cost of increasing communication (through the hidden constants in the asymptotic $O()$~term, which depends on~$\eps$).




% The proposed algorithm for coded \textsc{MBRB} facilitates an efficient and reliable broadcast that has strong delivery guarantees in the presence of Byzantine failures and the message adversary. 
% Via the use of erasure codes, cryptographic signatures, and the construction of Merkle trees~\cite{Merkle90}, the processes are able to gather quorums of signatures and coded message fragments.
% This allows the proposed solution to ensure reliable dissemination to a bounded minimum number, $\ell$, of receivers, as specified in Definition~\ref{def:mbrb}.

\medskip
The starting point of our algorithm is the AFRT algorithm~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}. This algorithm achieves all the desired MBRB properties (Definition~\ref{def:mbrb}), albeit with a large communication cost of at least $n^2|m|$ bits overall. 
This communication stems from the following approach: the sender disseminates the message $m$ to all nodes. However, the sender might be faulty and send different $m$'s to different nodes. 
The solution of the AFRT algorithm is that each node that receives a message from the sender signs it and forwards it to the entire network, along with its own signature and any other signature observed so far for that message.
The fact that each node re-broadcasts the message~$m$, by itself causes $n^2|m|$ bits of communication. 

In order to reduce the communication costs, we apply a coding technique, inspired by\remove{ an approach by} Alhaddad \etal~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}. Instead of communicating the message~$m$ directly, the sender first encodes the message using an error-correction code and ``splits'' the resulting codeword between the nodes, so that each node receives one fragment of size $O(|m|/n)$ bits.
Now, each node needs to broadcast only its fragment of the message rather than the entire message. This reduced per-node communication effectively reduces the overall communication for disseminating the message itself to $n|m|$ bits.

Due to the message adversary and the actions of the Byzantine nodes, some of the fragments might not arrive at their destination. 
However, the error-correction code has the property that the message~$m$ can be reconstructed from any sufficiently large subset of the fragments.
%
Byzantine nodes \ft{may, however, also propagate corrupt fragments. To protect honest nodes against this behavior
% can do even worse, namely, they can propagate an incorrect fragment. 
% Correct nodes cannot distinguish correct fragments from incorrect ones (at least, not until enough fragments are collected, and the message is reconstructed). Without this knowledge, the correct nodes might assist the Byzantine nodes in propagating incorrect fragments, harming the correctness of the algorithm.
%
% There are several ways to prevent the bad effects of such actions.
% The first option is to have the sender sign each fragment that it sends. When a node receives a fragment, the node could verify that the fragment is correctly signed by the sender, or ignore it otherwise. 
% The drawback of this solution is that only the sender can generate signatures for fragments. 
% In hindsight, in our MBRB algorithm, we rely on correct nodes that already reconstructed the correct message, to disseminate fragments of the message to those nodes that did not receive their fragment (say, due to the message adversary). In principle, when a node reconstructs the correct message, it can generate the codeword and obtain all the fragments, even if the node did not receive some of the fragments beforehand. However, the node cannot generate the sender's signature for the fragments it generated by itself. 
% Then, the node cannot relay these fragments to the other nodes. 
% This issue potentially leads to a reduced delivery power~$\ell$.
% The second option is to use a stronger code that can correctly reconstruct the message even if some of the fragments are corrupted. This solution is valid, however, it puts further constraints on the fraction of the  Byzantine nodes the MBRB algorithm can handle.
% We choose a different solution based on
the proposed algorithm exploits} Merkle trees~\cite{Merkle90},
\ft{which allow the sender to attach}
% Along with every fragment of the codeword, the sender attaches 
two pieces of information: the hash value $h$ of~$m$, and a \emph{proof of inclusion} for the fragment---a sequence of hash values that proves that the specific fragment is indeed a fragment of the message whose hash value is~$h$ (see \cref{sec:merkle} for detail).
\FT{I've removed an inroads on alternative solutions, and a comment saying that MTs are easy to construct.}%
% Given the message~$m$, it is easy to generate a proof of inclusion for any specific fragment.
% In particular, when a correct node succeeds in reconstructing~$m$, it can immediately generate the hash value~$h$, all the fragments, and all their respective proofs of inclusion.
% The node can then disseminate fragments (along with their proofs) and help other nodes to obtain enough fragments and reconstruct the message.

\ft{Finally, in order to prevent honest nodes from disseminating corrupt fragments and proofs before they can reconstruct a complete message,}
% The last remaining issue concerns the following question: How can we guarantee that only a single message~$m$, i.e., the message intended by the sender, is accepted by all nodes? 
% In AFRT, the sender signs the message~$m$ and sends both $m$ and its signature to all nodes. A node ignores any $m$ that is not correctly signed by the sender. 
% However, in our coded solution,
% none of the nodes can verify any signature of~$m$ before reconstructing it. 
% Again, nodes face the problem of being unable to distinguish correct fragments (i.e., fragments that belong to the \emph{sender}'s message $m$) from incorrect fragments. 
% The solution is immediate: instead of signing~$m$,
nodes sign the hash value~$h$, even without knowing~$m$. This\remove{ piece of information} is communicated along with every fragment, and further, the proof of inclusion holds with respect to that hash value. This means that Byzantine nodes cannot generate an incorrect fragment and a proof that will pass the verification, given the hash value~$h$ signed by \ft{a} correct sender. 

To complete the description of our MBRB algorithm, we mention that, similar to AFRT, our algorithm tries to form a quorum of signatures on some specific hash value $h$. In parallel, nodes collect fragments that verify as part of the message whose hash is~$h$. 
Once a node collects enough signatures (for some~$h$) and at the same time obtains enough message fragments that are proven to belong to the same~$h$, the node can reconstruct $m$ and deliver (accept) it. 
At this point, the node also disseminates the quorum of signatures along with (some of) the fragments. 
This allows other correct nodes to reconstruct the message and verify a quorum has been reached. 
In fact, the dissemination of fragments, including fragments that this node did not have before reconstructing the message, 
is a crucial step in amplifying the number of nodes that  deliver~$m$ to our stated level of $\ell=n-t-(1+\eps)\Dadv$.
See the full description of the MBRB algorithm in \cref{sec:MBRBscheme}.




\Subsection{Related work}
%
\emph{Byzantine reliable broadcast} (BRB) can be traced back to Pease, and Shostack, and Lamport~\cite{DBLP:journals/jacm/PeaseSL80}, which considered the particular case of synchronous message-passing systems.
Since then, solutions for reliable broadcast, together with the related \emph{consensus} problem, have been considered for many distributed systems~\cite{DBLP:books/sp/Raynal18}. 
In asynchronous systems, BRB solutions can be traced back to Bracha and Toueg~\cite{DBLP:conf/podc/BrachaT83,DBLP:journals/jacm/BrachaT85}.
Recent advances~\cite{DBLP:conf/srds/MaurerT14,DBLP:conf/opodis/GuerraouiKKPST20,DBLP:conf/icdcs/BonomiDFRT21,DBLP:conf/sss/DuvignauRS22} in Byzantine fault-tolerant (BFT) solutions to the problem of BRB include the above-mentioned \AFRT~\cite{DBLP:journals/corr/abs-2205-09992}, which safeguards also against \ft{a} message adversary \ft{capable of fully isolating some correct nodes}.
Our solution features substantially lower communication than \AFRT, without harming the other properties such as the total number of messages or the delivery power.

Computation in networks with link faults, namely, with Byzantine links was considered by Santoro and Widmayer~\cite{SW89,SW90}, who discussed various types of Byzantine actions, \eg combinations of omitting, corrupting, and injecting messages. 
The works of~\cite{DBLP:journals/tcs/SantoroW07,BDP97} focus on the case of reliable broadcast with such faults.
In~\cite{Pelc92}, Pelc proved that robust communication is feasible over graphs whose edge-connectivity is more than~$2f$, assuming the number of Byzantine links is bounded by~$f$.
This is also implied by the work of Dolev~\cite{Dolev82}. 
%
Censor-Hillel, Cohen, Gelles, and Sela~\cite{CCGS22} show that any computation can be performed when all links suffer arbitrary substitution faults (but no crashes), given that the network is 2-edge connected. 
When all links suffer corruption, but their overall amount is restricted, any computation can be reliably performed by Hoza and Schulman~\cite{HS16}, for synchronous networks where the topology is known, or by Censor-Hillel, Gelles, and Hauepler~\cite{CGH19}, for asynchronous networks with unknown topology.

The literature also deals with a setting that allows Byzantine nodes in addition to faulty links~\cite{PT86,gong1998byzantine,SCY98,Dasgupta98,biely03,DBLP:journals/tcs/BielySW11}.
% In particular, we note that Biely, Schmid, and Weiss~\cite{DBLP:journals/tcs/BielySW11} also consider a hybrid process and link failure model, but only in the context of synchronous message-passing systems, whereas this paper focuses specifically on asynchronous systems.
Building on~\cite{DBLP:journals/corr/abs-2205-09992}, the algorithm was also extended to signature-free asynchronous systems~\cite{DBLP:conf/opodis/AlbouyFRT22}, albeit with lower delivery guarantees, and a weaker resilience with respect to~$d$ and~$t$.
We consider fully connected \ta{asynchronous} networks, Byzantine nodes, and link failures that include only omissions. 
However, our \MBRB solution is the first, to the best of our knowledge, to offer a near-optimal communication (up to the length of the signature, $\kappa$) and delivery power~$\ell$.

%\FT{I would suggest using `faulty links' in the previous sentence, as some of these refs (e.g.~\cite{gong1998byzantine}) only consider omission faults on their links: in the model of~\cite{gong1998byzantine} a message might not arrive on a faulty link, in which case an error is detected.}%%
%\FT{I'm not sure we should include \cite{PT86}. This paper considers a model in which faulty processes might omit to send or receive messages (omission faults) but do not act arbitrarily (are not Byzantine). Faults are also pinned to specific processes (rather than `mobile' as with a message adversary). If we do include \cite{PT86}, we should not suggest it combines Byzantine nodes and Byzantine links.}


Coding techniques are implemented to minimize the dissemination costs associated with message transmission across the network, ensuring the ability to reconstruct data in the event of\remove{ node} failures or adversarial compromises.
In the context of Blockchains, significant contributions have been made by Cachin and Tessaro~\cite{DBLP:conf/wdag/CachinT05a} as well as Cachin and Poritz in SINTRA~\cite{DBLP:conf/dsn/CachinP02}, followed by its successors such as HoneyBadgersBFT~\cite{DBLP:conf/ccs/MillerXCSS16}, BEAT~\cite{DBLP:conf/ccs/DuanRZ18}, and Alhaddad \etal~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}.
These solutions leverage digital signatures and coding techniques to provide a balanced and reliable broadcast.
Our work contributes to advancing\remove{ the state of the art in} the field of coded reliable broadcast by offering improved fault-tolerance guarantees that are stronger than the aforementioned solutions.

%\ran{need to mention the gradecast of Abraham and Asharov, which also uses coding technique and has some similarities in ideas to us}

%Specifically, we address the challenge posed by a combined adversary that possesses control over both $t$ out of $n$ Byzantine nodes and the message transmission mechanism.
%This adversary has the ability to selectively omit up to $d$ out of $n$ messages during each broadcast initiated by a non-faulty node.  

%\ran{IMHO, this section is still too long and maybe not really adequate for the topic. I tried to cut it a bit but maybe more effort is due}
%\ran{who are the relevant reviewers for this work? Are we citing their related works?}


==> sec-intro_initial.tex <==

\Section{Introduction}
%	
\emph{Reliable Broadcast} allows $n$ asynchronous nodes to agree eventually on a message sent by a designated node, the \emph{sender}, despite the possible malicious behavior by some\reduce{ of the} nodes and the transmission network. 
Reliable broadcast plays a crucial role in several key applications, including consensus algorithms, replication, event notification, and distributed file systems, among others.
These systems sometimes require broadcasting large messages or files (\eg permissioned blockchains), and thus, reducing the communication overhead to a minimum is an important aspect of achieving scalability.
% \FT{We could also mention, in 
% which blocks can be quite large (although, admittedly, some approaches have been proposed to decouple agreement on a block from its diffusion, e.g. in HoneyBadger.).}
% \TA{Yes but as we have seen before, sending the whole message and r-broadcasting the hash of this message at the same time 2 is not optimal for our case, because it gives a delivery power of $c-2d$. Maybe HoneyBadger would have the same problem of weak termination guarantees if there was an MA.}
In that vein, this work aims at providing \emph{communication efficient} solutions for the task of reliable broadcast in the presence of node and link faults.
%\TA{I would replace "consistency guarantees" with "fault-tolerance guarantees". The consistency guarantees stay the same (it is still a reliable broadcast), but the fault-tolerance guarantees get stronger (MA+Byz), no?}
%\ran{IMHO, it is too early to reach this point here. What fits here is a (vague) statement that our focus is BRB and reducing its communication. the rest should appear later. I changed accordingly}

%
%(e.g., in the case of broadcast-based distributed file systems), 

\emph{Byzantine} nodes~\cite{Dolev82,LSP82} are faulty processes that are assumed to act cooperatively in an arbitrary manner to hinder the non-faulty nodes (also known as correct nodes) from reaching an agreement on the value of a sent message.
These faulty nodes can manifest in various ways, such as delivering fake messages that were never sent, altering the payload of messages sent by any faulty nodes, delaying message delivery, or even omitting messages altogether. Also, a Byzantine failure can present itself differently to different nodes.

Solving reliable broadcast in the presence of Byzantine nodes (a problem known as BRB for Byzantine Reliable Broadcast~\cite{B87}) has been extensively studied for at least four decades. Bracha~\cite{DBLP:conf/podc/BrachaT83,DBLP:journals/jacm/BrachaT85} in particular showed that BRB could be implemented in asynchronous networks as soon as the number $t$ of Byzantine nodes is limited to be less than a third of the nodes. This seminal result has since been followed by hundreds of works, with a various range of optimizations and tradeoffs between different parameters such as resilience, efficiency, and communication; see~\cite{DBLP:books/sp/Raynal18} for an excellent book on this topic.

A significant challenge to reliable broadcast algorithms arises when the message-passing system is unreliable and possibly cooperates with the Byzantine nodes. Link faults~\cite{SW89,DBLP:journals/tcs/SantoroW07} give Byzantine nodes (potentially limited) control over certain network links, enabling them to omit or corrupt messages \ft{(an ability captured under the umbrella term \emph{message adversary}~\cite{DBLP:reference/algo/Raynal16a})}.
This work focuses on a specific type of \emph{message adversary}~\cite{DBLP:reference/algo/Raynal16a} that can only omit messages sent by correct nodes, but that cannot alter their content. 
This message adversary abstracts cases related to \emph{silent churn}, where nodes may voluntarily or involuntarily disconnect from the network without explicitly notifying other nodes. 
During disconnection, the adversary causes correct nodes to pause the execution of their algorithm temporarily and resume upon reconnecting. 
In the message adversary model, correct nodes may miss messages sent over reliable communication channels by other nodes while they are disconnected, as there is no explicit notification about the message omission.

\EMS{Rev. \#3 left a comment '- Having finished the paper, I would have liked to see a little more discussion comparing this paper's result and the $\Omega$($n|m| + n^2\kappa$) "straightforward lower bound" discussed just before Section 1.1. If I understand correctly, there's an extra $n$ factor on the $\kappa$ term that the present algorithm uses, and I'd like to understand if the authors think this necessary.'}%



\Subsection{Problem \ft{overview}}%description}
%
\label{sec:probDesc}
%
%We briefly describe the setting and problem of reliable broadcast, see \cref{sec:prelim} for further details.
We assume $n$ nodes over an asynchronous network, where a message can be delayed for an arbitrary yet finite amount of time (unless omitted by the message adversary). 
\FT{PLEASE CHECK. I've moved up the description of the MA. In the previous version, we mentioned the $\comm$ primitive before defining it.}%
We assume the existence of $t$ Byzantine nodes and a message adversary %that can omit up to $d$ messages per invocation of the $\comm$ primitive. 
\ft{%
capable of omitting up to~$d$ messages per node's broadcast. 
To be more precise, a node communicates through a $\comm$ primitive (or a similar multicast/unicast primitive that targets a dynamically defined subset of processes),
which results in the transmission of~$n$ messages, with each node being sent one message, including the sender.
The message adversary can choose to omit messages in transit to a subset of at most $d$ correct processes.
The adversary is only limited by the size of that subset.
For instance, between different $\comm$ invocations, the adversary has the freedom to modify the set of correct processes to which messages are omitted.
}%
Furthermore, a designated sender node holds a message $m$ that it wishes to broadcast to all the nodes. 

An algorithm that satisfies the requirements of reliable broadcast despite Byzantine nodes and a message adversary is called a \emph{Message-adversary Byzantine Reliable Broadcast} (\MBRB) algorithm.
The detailed version of \MBRB's requirements was formulated in~\cite{AFRT23}, see \cref{sec:MBRBdef}.
\rane{We informally summarize them here as follows.
\textbf{(1)} For any sender invoking the broadcast algorithm, no two correct nodes deliver $m$ and $m'$, such that $m'\ne m$.
\textbf{(2)} 
%If a correct sender broadcasts a message~$m$, 
For any sender invoking the broadcast algorithm,
either zero or at least $\ell$ correct nodes will deliver~$m$.
The quantity $\ell$ might depend on the adversary's power, \ie on $t$ and~$d$.
\textbf{(3)} If a correct node delivers some message~$m$ from a \emph{correct sender}, this correct sender has broadcast $m$ previously and at least $\ell$ correct nodes will deliver it.
}

\Subsection{Background}
%
\label{sec:backGround}
%
Albouy, Frey, Raynal, and Taïani~\cite{AFRT23} recently proposed a \ft{Message-adversary Byzantine} Reliable Broadcast algorithm (which we denote \AFRT for short) for asynchronous networks that withstands the presence of $t$ Byzantine nodes and a message adversary capable of omitting up to $d$ messages per node’s broadcast.
\AFRT guarantees the reliable delivery of any message when $n>3$t+$2d$. 
Moreover, they demonstrate the necessity of this bound on the number of Byzantine nodes and omitted messages, as no reliable broadcast algorithm exists otherwise.

% \EMS{Please see the first comment from reviewer \#1 asking whether it should be O(nm+nk) or $O(nm+n^2k)$. The reviewer also say 'in case the former is true, mention that you get an improvement only when m is longer than kn.'}%
% \FT{The latter is true. $O(nm+n^2\kappa)$ is correct.}
% %
% \EMS{Ran, can you help to unify the text?}
% \ran{I agree with Francois' correction. Elad, what is here to unify?}
% %

One caveat of \AFRT regards its communication efficiency. 
While it achieves an optimal number of $\bigO{n^2}$ messages, \ft{and an optimal delivery power $\ell=n-t-d$}, each node's communication requires $\bigO{n\cdot(|m|+\ft{n}\kappa)}$ bits, where $|m|$ represents the number of bits in the broadcast message 
%$\log n$ corresponds to the size of a node identity, 
and $\kappa$ is the length of the digital signatures used in their algorithm. 
In the current work, we design an algorithm that significantly reduces the communication cost per node while preserving the total number of messages communicated.  
Our solution features at most~$4n$ messages \ft{per correct node (corresponding to $4n^2$ messages overall)}, and only $\bigO{|m| + n^2\kappa}$ bits per \ta{correct }node.
Overall, $\bigO{n|m| + n^3\kappa}$ bits are communicated \ta{by correct nodes}.
\rane{Reducing the second term to $(n^2\log n)\kappa$ can be done by employing standard techniques of \emph{threshold signatures}, which replace the need to communicate a quorum of signatures; see, e.g.,~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}.}
Note that $\Omega$($n|m| + n^2\kappa$) is a straightforward lower bound on the overall communication \ft{for deterministic algorithms using signatures} (up to the size of the signature), see\reduce{ \eg} \cite{DBLP:conf/ccs/DasX021,nayak_et_al:LIPIcs:2020:13106}, as every \ta{correct} node must receive the message~$m$, and as the reliable broadcast of a single bit necessitates at least $\Omega$($n^2$) messages~\cite{DR85}.

\EMS{Comments from Reviewer \#1. '-Isn't it true that AFRT get a better value for $\ell$, i.e., they do not lose the eps? If this is indeed the case, this should be highlighted (and in any case a comparison should be made.)'}%
%\FT{Do we want to mention the reduced $\ell$ here, or at least hint as it, e.g. `a slightly reduced delivery power'? We haven't discussed delivery power yet, and the information comes just below in Sec 1.3.}
%



%\vspace*{-1em}
\Subsection{Contributions and techniques}
%	
\ft{This paper is the first to} present a \MBRB algorithm \ft{able to tolerate an hybrid adversary combining $t$ Byzantine nodes and a Message Adversary of power $d$, while providing} \ft{optimal Byzantine resilience,} near-optimal communication, and \ft{near-optimal} delivery power~$\ell$.
\B\begin{theorem}[Main, informal]
\label{thm:main-informal}
For any~$\eps>0$, there exists an efficient \MBRB algorithm, such that every message~$m$ broadcast via this scheme is delivered by at least $\ell = n-t-(1+\eps)d$ correct nodes \ft{under the assumption $n>3t+2d$}. 
Each correct node sends  no more than $4n$ messages and communicates 
$\bigO{|m|+n^2\kappa}$ bits overall, where $|m|$ is the length of the message~$m$. 
\end{theorem}
\B




%We note that 
The above asymptotic communication complexity holds assuming a sufficiently long message~$m$. 
Further,\reduce{ we note that} $n-t-\Dadv$ is a natural upper bound on the delivery power~$\ell$ of any MBRB algorithm. This bound arises from the power of the message adversary to isolate a subset of the correct parties of size~$\Dadv$, and omit all messages sent to this subset. 
Our solution obtains a delivery power~$\ell$  that is as close to the limit as desired, at the cost of increasing communication (through the hidden constants in the asymptotic $\bigO{\cdot}$~term, which depends on~$\eps$).
\ft{Finally, $n>3t+2d$ is a necessary condition to implement MBRB under asynchrony~\cite{DBLP:conf/opodis/AlbouyFRT22}, thus making our solution optimal in terms of Byzantine resilience.}



% The proposed algorithm for coded \textsc{MBRB} facilitates an efficient and reliable broadcast that has strong delivery guarantees in the presence of Byzantine failures and the message adversary. 
% Via the use of erasure codes, cryptographic signatures, and the construction of Merkle trees~\cite{Merkle90}, the processes are able to gather quorums of signatures and coded message fragments.
% This allows the proposed solution to ensure reliable dissemination to a bounded minimum number, $\ell$, of receivers, as specified in Definition~\ref{def:mbrb}.

%\medskip
The starting point of our algorithm is the AFRT algorithm~\cite{AFRT23}. This algorithm achieves all the desired MBRB properties (Definition~\ref{def:mbrb}), albeit with a large communication cost of at least $n^2|m|$ bits overall. 
This communication \ft{cost stems from the re-emission strategy used by AFRT. In the AFRT algorithm, the sender first disseminates the message $m$ to all nodes. To counter a possibly faulty sender, each node that receives $m$ signs it and forwards it to the entire network, along with its own signature and any other signature observed so far for that message. This re-broadcasting step leads to  $n^2|m|$ bits of communication.}


% stems from the following approach: the sender disseminates the message $m$ to all nodes. However, the sender might be faulty and send different $m$'s to different nodes. 
% The solution of the AFRT algorithm is that each node that receives a message from the sender signs it and forwards it to the entire network, along with its own signature and any other signature observed so far for that message.
% The fact that each node re-broadcasts the message~$m$, by itself causes $n^2|m|$ bits of communication. 

In order to reduce the communication costs,  we apply a coding technique, inspired by an approach by Alhaddad \etal~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}. Instead of communicating the message~$m$ directly, the sender first encodes the message using an error-correction code and ``splits'' the resulting codeword between the nodes, so that each node receives one fragment of size $\bigO{|m|/n}$ bits.
Now, each node needs to broadcast only its fragment of the message rather than the entire message. This reduced per-node communication effectively reduces the overall communication for disseminating the message itself to $n|m|$ bits.

Due to the message adversary and the actions of the Byzantine nodes,
some of the fragments might not arrive at their
destination. Error-correction codes have the property that the
message~$m$ can be reconstructed from any sufficiently large subset of
the fragments.  But Byzantine nodes can do even worse, namely, they
can propagate an incorrect fragment. Correct nodes cannot distinguish
correct fragments from incorrect ones (at least, not until enough
fragments are collected, and the message is reconstructed). Without
this knowledge, correct nodes might assist the Byzantine nodes in
propagating incorrect fragments, \ft{possibly} harming the correctness \ft{and/or performance} of the
algorithm.  To prevent this, the sender could sign each fragment that
it sends. A node that receives a fragment could then verify that the
fragment is correctly signed by the sender, and could ignore it
otherwise.  The drawback of this solution is that only the sender can
generate signatures for fragments.

In our MBRB algorithm, we rely on correct nodes that have already
reconstructed the correct message to disseminate its fragments to the
nodes that have not received any (say, due to the message
adversary). In principle, when a node reconstructs the correct
message, it can generate the codeword and obtain all the fragments,
even if the node did not receive some of the fragments
beforehand. However, the node cannot generate the sender's signature
for the fragments it generated by itself.  Because of this, the node
cannot relay these fragments to the other nodes, which potentially
leads to a reduced delivery power~$\ell$.  
\FT{PLEASE CHECK YOU AGREE: I am removing the following sentence, as corrupted fragments can be tolerated (with a strong enough code that tolerates corruptions) without reducing the Byzantine resilience using the \emph{Online-Error-Correction} (OEC) mechanism introduced by Ben-Or, Canetti, and Goldreich, as explained in \cite{DBLP:conf/podc/AlhaddadDD0VXZ22} by Alhaddad \etal. I am adding a footnote to mention this approach (as an alternative to signed Merkle proofs) and why we do not follow it.
The deleted sentence:
`%
A stronger code that can
correctly reconstruct the message even if some of the fragments are
corrupted could mitigate this issue, but it would put further
constraints on the fraction of the Byzantine nodes the MBRB algorithm
can handle.%
'}

\FT{We should not say the solution is novel, as signed Merkle trees have been proposed before, particularly in \cite{DBLP:conf/wdag/CachinT05a}.}
We, therefore, reuse \ft{the solution proposed by Cachin and Tessaro in \cite{DBLP:conf/wdag/CachinT05a}} and exploit Merkle
trees~\cite{Merkle90}. Along with every fragment of the
codeword, the sender attaches two pieces of information: the hash
value $h$ of~$m$, and a \emph{proof of inclusion} for the fragment---a
sequence of hash values that proves that the specific fragment is
indeed a fragment of the message whose hash value is~$h$ (see
\cref{sec:merkle} for detail).  Given the message~$m$, it is easy to
generate a proof of inclusion for any specific fragment.  In
particular, when a correct node succeeds in reconstructing~$m$, it can
immediately generate the hash value~$h$, all the fragments, and all
their respective proofs of inclusion.  The node can then disseminate
fragments (along with their proofs), help other nodes obtain
enough fragments, and reconstruct the message.%
\footnote{\ft{An alternative to Merkle proofs could be to use the Online-Error-Correction (OEC) protocol of Ben-Or, Canetti, and Goldreich~\cite{DBLP:conf/stoc/Ben-OrCG93}. Using a Reed-Solomon code~\cite{RS60}, OEC can eventually reconstruct the initial message $m$ without signatures~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}. However, because our solution requires the dissemination of quorums of signatures, the gain in terms of communication cost would be limited.%
\FT{PLEASE CHECK.}%
}} 

%The last remaining issue concerns the following question: How can we guarantee that only a single message~$m$, i.e., the message intended by the sender, is accepted by all nodes? 

The last issue concerns the following: How to guarantee that a single message~$m$, \ie the message intended by the sender, is accepted by all nodes? 
In AFRT, the sender signs the message~$m$ and sends both $m$ and its signature to all nodes. A node ignores any $m$ incorrectly signed by the sender. 
However, in our coded solution,
none of the nodes can verify any signature of~$m$ before reconstructing it. 
Again, nodes face the problem of being unable to distinguish correct fragments (\ie fragments that belong to the \emph{sender}'s message $m$) from incorrect fragments. 
The solution is immediate: instead of signing~$m$, nodes sign the hash value~$h$, even without knowing~$m$. This piece of information is communicated along with every fragment, and further, the proof of inclusion holds with respect to that hash value. This means that Byzantine nodes cannot generate an incorrect fragment and a proof that will pass the verification, given the hash value~$h$ signed by the correct sender. 

To complete the description of our MBRB algorithm, we mention that, similar to AFRT, our algorithm tries to form a quorum of signatures on some specific hash value $h$. In parallel, nodes collect fragments that they verify as part of the message whose hash is~$h$. 
Once a node collects enough signatures (for some~$h$) and at the same time obtains enough message fragments that are proven to belong to the same~$h$, the node can reconstruct~$m$ and deliver (accept) it. 
At this point, the node also disseminates the quorum of signatures along with (some of) the fragments. 
This allows other correct nodes to reconstruct the message and verify a quorum has been reached. 
In fact, the dissemination of fragments, including fragments that this node did not have before reconstructing the message, 
is a crucial step in amplifying the number of nodes that  deliver~$m$ to our stated level of $\ell=n-t-(1+\eps)\Dadv$.
See the full description of the MBRB algorithm in \cref{sec:MBRBscheme}.
%
\EMS{Rev. \#1 says about the above: 'You mention the alternative approach of using error correction - how does it affect the resiliency threshold in comparison to the MT solution?'}%
%

\ft{Although our algorithm builds quorums on hash values, it departs substantially from the communication-optimal BRB algorithm proposed by Das, Xiang, and Ren~\cite{DBLP:conf/ccs/DasX021}, which avoids signatures and relies on hashes only. The solution proposed in~\cite{DBLP:conf/ccs/DasX021} delivers a communication complexity in $O(n|M|+\kappa n^2)$ that is optimal up to the $\kappa$ parameter. Following initial dissemination of the message $m$ by the sender, their proposal runs Bracha's algorithm on the hash value of the broadcast message to ensure agreement. Unfortunately, when used with a message adversary, Bracha's algorithm loses the sub-optimal Byzantine resilience $n>3t+2d$ that AFRT and our solution provide, which is the reason why the solution presented in this paper avoids it. (See \cref{sec:Bracha:with:MA} for a more detailed discussion of why this is so.)}

\Fs
Due to the page limit, the complete analysis and proof details appear in the Appendix. 


\Subsection{Related work}
%
\emph{Byzantine reliable broadcast} (BRB) can be traced back to Pease, Shostak, and Lamport~\cite{DBLP:journals/jacm/PeaseSL80}, which considered the particular case of synchronous message-passing systems.
Since then, solutions for reliable broadcast, together with the related \emph{consensus} problem, have been considered for many distributed systems~\cite{DBLP:books/sp/Raynal18}. 
In asynchronous systems, BRB solutions can be traced back to Bracha and Toueg~\cite{DBLP:conf/podc/BrachaT83,DBLP:journals/jacm/BrachaT85}.
Recent advances~\cite{DBLP:conf/srds/MaurerT14,DBLP:conf/opodis/GuerraouiKKPST20,DBLP:conf/icdcs/BonomiDFRT21,DBLP:conf/sss/DuvignauRS22} in Byzantine fault-tolerant (BFT) solutions to the problem of BRB include the above-mentioned \AFRT~\cite{AFRT23}, which safeguards also against the message adversary.
Our solution features substantially lower communication than \AFRT, without harming the other properties, \eg the\reduce{ total} number of messages or the delivery power.

Computation in networks with link faults, namely, with Byzantine links was considered by Santoro and Widmayer~\cite{SW89,SW90}, who discussed various types of Byzantine actions, \eg omitting messages, corrupting messages, injecting messages, and combinations thereof. 
The works of~\cite{DBLP:journals/tcs/SantoroW07,BDP97} focus on the case of reliable broadcast with such faults.
In~\cite{Pelc92}, Pelc proved that robust communication is feasible over graphs whose edge-connectivity is more than~$2f$, assuming the number of Byzantine links is bounded by~$f$.
This is also implied by the work of Dolev~\cite{Dolev82}. 
%
Censor-Hillel, Cohen, Gelles, and Sela~\cite{CCGS22} show that any computation can be performed when all links suffer arbitrary substitution faults (but no crashes), given that the network is 2-edge connected. 
When all links suffer corruption, but their overall amount is restricted, any computation can be reliably performed by Hoza and Schulman~\cite{HS16}, for synchronous networks where the topology is known, or by Censor-Hillel, Gelles, and Haeupler~\cite{CGH19}, for asynchronous networks with unknown topology.

Settings that allow Byzantine nodes in addition to faulty links were considered~\cite{PT86,gong1998byzantine,SCY98,Dasgupta98,biely03,DBLP:journals/tcs/BielySW11}.
Building on~\cite{AFRT23}, the algorithm was also extended to signature-free asynchronous systems~\cite{DBLP:conf/opodis/AlbouyFRT22}, albeit with lower delivery guarantees, and a weaker resilience with respect to~$d$ and~$t$.
We consider fully connected \ta{asynchronous} networks, Byzantine nodes, and omission only link failures. 
But, our \MBRB is the first, to the best of our knowledge, to offer a near-optimal communication (up to the length of the signature, $\kappa$) and delivery power~$\ell$.

% In particular, we note that Biely, Schmid, and Weiss~\cite{DBLP:journals/tcs/BielySW11} also consider a hybrid process and link failure model, but only in the context of synchronous message-passing systems, whereas this paper focuses specifically on asynchronous systems.

%\FT{I would suggest using `faulty links' in the previous sentence, as some of these refs (e.g.~\cite{gong1998byzantine}) only consider omission faults on their links: in the model of~\cite{gong1998byzantine} a message might not arrive on a faulty link, in which case an error is detected.}%%
%\FT{I'm not sure we should include \cite{PT86}. This paper considers a model in which faulty processes might omit to send or receive messages (omission faults) but do not act arbitrarily (are not Byzantine). Faults are also pinned to specific processes (rather than `mobile' as with a message adversary). If we do include \cite{PT86}, we should not suggest it combines Byzantine nodes and Byzantine links.}


Coding techniques are implemented to minimize the dissemination costs associated with message transmission across the network, ensuring the ability to reconstruct data in the event of node failures or adversarial compromises.
In the context of Blockchains, significant contributions have been made by Cachin and Tessaro~\cite{DBLP:conf/wdag/CachinT05a} as well as Cachin and Poritz in SINTRA~\cite{DBLP:conf/dsn/CachinP02}, followed by its successors such as HoneyBadgersBFT~\cite{DBLP:conf/ccs/MillerXCSS16}, BEAT~\cite{DBLP:conf/ccs/DuanRZ18}, DispersedLedger~\cite{DBLP:conf/nsdi/YangPAKT22} and Alhaddad \etal~\cite{DBLP:conf/podc/AlhaddadDD0VXZ22}.
These solutions leverage digital signatures and coding techniques to provide a balanced and reliable broadcast.
Our work contributes to the advancement of the state of the art in the field of coded reliable broadcast by offering improved fault-tolerance guarantees that are stronger than the aforementioned solutions.

%\ran{need to mention the gradecast of Abraham and Asharov, which also uses coding technique and has some similarities in ideas to us}

%Specifically, we address the challenge posed by a combined adversary that possesses control over both $t$ out of $n$ Byzantine nodes and the message transmission mechanism.
%This adversary has the ability to selectively omit up to $d$ out of $n$ messages during each broadcast initiated by a non-faulty node.  

%\ran{IMHO, this section is still too long and maybe not really adequate for the topic. I tried to cut it a bit but maybe more effort is due}
%\ran{who are the relevant reviewers for this work? Are we citing their related works?}

